K-Nearest Oracles Borderline Dynamic Classifier Ensemble Selection

Dynamic Ensemble Selection (DES) techniques aim to select locally competent classifiers for the classification of each new test sample. Most DES techniques estimate the competence of classifiers using a given criterion over the region of competence of the test sample (its the nearest neighbors in the validation set). The K-Nearest Oracles Eliminate (KNORA-E) DES selects all classifiers that correctly classify all samples in the region of competence of the test sample, if such classifier exists, otherwise, it removes from the region of competence the sample that is furthest from the test sample, and the process repeats. When the region of competence has samples of different classes, KNORA-E can reduce the region of competence in such a way that only samples of a single class remain in the region of competence, leading to the selection of locally incompetent classifiers that classify all samples in the region of competence as being from the same class. In this paper, we propose two DES techniques: K-Nearest Oracles Borderline (KNORA-B) and K-Nearest Oracles Borderline Imbalanced (KNORA-BI). KNORA-B is a DES technique based on KNORA-E that reduces the region of competence but maintains at least one sample from each class that is in the original region of competence. KNORA-BI is a variation of KNORA-B for imbalance datasets that reduces the region of competence but maintains at least one minority class sample if there is any in the original region of competence. Experiments are conducted comparing the proposed techniques with 19 DES techniques from the literature using 40 datasets. The results show that the proposed techniques achieved interesting results, with KNORA-BI outperforming state-of-art techniques.

==> content/chapters/chapter-1/old-chapter-1.tex <==

\section{Introduction}
% no \PARstart

	Supervised learning is the machine learning task of classifying unlabeled samples of data into classes, based on a training set of class labeled samples. The nearest neighbor (NN) rule \cite{nnpc:1967} is one of the most well known supervised learning techniques. The general idea is to classify a new instance as being of the same class as the nearest instance from the training set. The K-nearest neighbor rule (KNN) \cite{knnrule:1969} is a generalization of the NN rule that considers the label of the K nearest instances of an unknown instance to make the classification. This technique is very simple, yet is one of the most interesting and useful algorithms in Pattern Recognition \cite{Shakhnarovich:2006}.

	Despite the high classification accuracy, the KNN has several drawbacks \cite{Kononenko:2007:MLD:1535465}, the three most relevant are:
\begin{enumerate}
\item \textbf{high storage requirements}: the KNN needs to store all training set, because the decision rule is defined by all training instances.
\item \textbf{low time of response}: for every new classification, the KNN needs to visit all instances from the training set ($\mathcal{O}(n)$ complexity, where $n$ is the size of the traning set).
\item \textbf{low tolerance to noise}: the KNN considers all data from the training set to be relevant to the classification task. Because of that, noisy data might compromise the classification accuracy.
\end{enumerate}

	In the literature, many approaches were proposed to solve these issues \cite{approaches:2008}. A successful approach that handles those drawbacks of the KNN is the use of instance reduction \cite{hybrid:2000}. Techniques of instance reduction aim to select only relevant instances from the training set, creating a smaller training set without compromising the classification accuracy \cite{hybrid:2000}. In doing so, the storage requirements and time of response are reduced, because less instances are saved and visited in each classification, and also removes noisy data, improving classification and solving the noise sensitivity problem.

	Prototype selection (PS) is a process of instance reduction that removes instances that are redundant or irrelevant to the classification, and selects the representative ones. Prototype generation (PG) is the process of instance reduction that generates artificial instances in order to achieve a higher generalization and create a more suitable training set. Because of the limitations of the search space of PS techniques, PG techniques have the potential of achieve a higher reduction rate than PS techniques. 

	Evolutionary algorithms (EAs) have been successfully used in several machine learning problems. The use of EAs to solve PS problems is called evolutionary prototype selection (EPS) and it has been achieving interesting results \cite{epsstudy}. Until the date, the most well know instance reduction technique is the Steady-State Memetic Algorithm (SSMA), an EPS technique that uses a local search to find the optimal solution. 

Despite the high performance of instance reduction in general, even the most advanced techniques have drawbacks when dealing with some specific types of datasets. Some datasets have many instances of one class, the majority class, and only a few of the other, the minority class. Learning from such datasets is a difficult task, being considered one of the top 10 problems of data mining and pattern recognition \cite{10problemsInDM:2006}.

	The problem of instance reduction techniques with imbalanced datasets is that, usually, these techniques select many instances of the majority class and only a few, of even none, of the minority class \cite{asgp:2012}. The reason for such behavior is that the minority class instances are considered as noise, and sometimes, considered as outliers that need to be removed in order to improve generalization. This is a problem because the minority class is usually the one that carries the concept to be learnt, like medical diagnostics applications \cite{conf/icml/HulseKN07}).

	The use of oversampling and pre-processing techniques, such as One-Sided Selection \cite{oss:2000}, have been successfully applied to these algorithms, but only a few are self contained to handle this issue. Some techniques with a high performance of classification when trained with regular datasets have a low performance when trained with imbalanced datasets.

In \cite{asgp:2012}, the authors showed that the \textit{Self-Generating Prototypes} (SGP) \cite{sgp:2007}, one of the most efficient centroid-based PG techniques, has a low performance when dealing with imbalanced datasets. The \textit{Adaptive Self-Generating Prototypes} (ASGP) \cite{asgp:2012} was proposed in order to solve this issue, and achieved impressive results when compared to the previous version of the SGP. The problem with the ASGP is that, when improving the classification accuracy, the reduction rate is reduced, becoming equivalent to the SGP and worst than the SGP2.

This paper proposes an architecture composed by two algorithms: incremental merging and evolutionary pruning. The proposed algorithms can be combined with any PG algorithm, in order to improve its performance. The incremental merging expands the search space inserting new generalized samples that might better represent the distribution of classes. The evolutionary pruning is a memetic algorithm (MA) based on the SSMA used to explore the search space and find optimal solution. The evolutionary pruning uses the original training set as a validation set, instead of using the new generated samples.

In the experiments, the we combined the proposed steps with the ASGP, proposing the \textit{Evolutionary Adaptive Self-Generating Prototypes} (EASGP), and concluded that both, classification accuracy and reduction ratio, were improved in comparision to previous versions of the SGP algorithm.

This paper is organized as follows. A review of instance reduction techniques, as well as related work on evolutionary algorithms, are given in Section II. Section III presents the proposed algorithms. In Section IV, the experiments are presented and the results are analysed. Finally, Section V concludes the paper.


==> content/chapters/chapter-2/fig-all.tex <==


\begin{figure*}[ht]
\centering
\subfigure[Artificial Dataset 1]{
	\includegraphics[width=2.2in]{images/examples/case1/ARTIFICIAL_ORIG.eps}
    \label{subfig:1}
}
\subfigure[SGP2 over Artificial Dataset 1]{
	\includegraphics[width=2.2in]{images/examples/case1/ARTIFICIAL_SGP2.eps}
    \label{subfig:2}
}
\subfigure[ASGP over Artificial Dataset 1]{
	\includegraphics[width=2.2in]{images/examples/case1/ARTIFICIAL_ASGP.eps}
    \label{subfig:3}
}
\subfigure[Artificial Dataset 2]{
	\includegraphics[width=2.2in]{images/examples/case2/ARTIFICIAL_ORIG.eps}
    \label{subfig:4}
}
\subfigure[SGP2 over Artificial Dataset 2]{
	\includegraphics[width=2.2in]{images/examples/case2/ARTIFICIAL_SGP2.eps}
    \label{subfig:5}
}
\subfigure[ASGP over Artificial Dataset 2]{
	\includegraphics[width=2.2in]{images/examples/case2/ARTIFICIAL_ASGP.eps}
    \label{subfig:6}
}
\subfigure[Artificial Dataset 3]{
	\includegraphics[width=2.2in]{images/examples/case3/ARTIFICIAL_ORIG.eps}
    \label{subfig:7}
}
\subfigure[SGP2 over Artificial Dataset 3]{
	\includegraphics[width=2.2in]{images/examples/case3/ARTIFICIAL_SGP2.eps}
    \label{subfig:8}
}
\subfigure[ASGP over Artificial Dataset 3]{
	\includegraphics[width=2.2in]{images/examples/case3/ARTIFICIAL_ASGP.eps}
    \label{subfig:9}
}
\caption{Artificial Datasets}
\label{fig:artificialall}
\end{figure*}



==> content/chapters/chapter-2/fig-sgp2.tex <==

\begin{figure}[ht]
\centering
\subfigure[Artificial Dataset 1]{
%	\includegraphics[width=2in]{images/examples/case1/ARTIFICIAL_ORIG.eps}
	\includegraphics[width=4cm,height=3cm]{images/examples/case1/ARTIFICIAL_ORIG.eps}
%    \rule{4cm}{3cm}
    \label{subfig:o11}
}
\subfigure[SGP2 over Artificial Dataset 1]{
%	\includegraphics[width=2in]{images/examples/case1/ARTIFICIAL_SGP2.eps}
	\includegraphics[width=4cm,height=3cm]{images/examples/case1/ARTIFICIAL_SGP2.eps}
%    \rule{4cm}{3cm}
    \label{subfig:sgp21}
}
\subfigure[Artificial Dataset 2]{
%	\includegraphics[width=2in]{images/examples/case2/ARTIFICIAL_ORIG.eps}
	\includegraphics[width=4cm,height=3cm]{images/examples/case2/ARTIFICIAL_ORIG.eps}
%    \rule{4cm}{3cm}
    \label{subfig:o12}
}
\subfigure[SGP2 over Artificial Dataset 2]{
%	\includegraphics[width=2in]{images/examples/case2/ARTIFICIAL_SGP2.eps}
	\includegraphics[width=4cm,height=3cm]{images/examples/case2/ARTIFICIAL_SGP2.eps}
%    \rule{4cm}{3cm}
    \label{subfig:sgp22}
}
\caption{Artificial Datasets and SGP2 Generated Prototypes}
\label{fig:artificialsgp2}
\end{figure}



==> content/chapters/chapter-3/sts.chapter-3.tex <==
\section{Problem Statement}
\label{sec:problem_statement}

When no classifier correctly classifies all samples in the region
of competence of a test sample, KNORA-E reduces the region of competence
by removing the sample that is further away from $x_{query}$, regardless of its class.
Because of that, KNORA-E can change a region of competence
that is composed of samples from different classes into a region of
competence composed of samples of a single class.

Figure \ref{fig:kne} presents the iterations of KNORA-E ($K = 5$)
for the classification of a test sample ($x_{query}$) when no
classifier correctly classifies all samples in the region of
competence ($\Psi$) of $x_{query}$.
In this figure, $\blacktriangle$ is the test sample,
the dotted line delimits the region of competence,
$A$, $B$, $C$, $D$, and $E$ are the $K$ nearest neighbors of
$x_{query}$ in the validation set,
$c1$ and $c2$ are classifiers and
the continuous straight lines are their decision boundaries.
The markers $\bluecircle$ and $\redsquare$ represent samples from different classes,
and the test sample is from the class "$\bluecircle$".

\begin{figure*}[!hbtp]
\begin{center}
    \subfloat[1st iteration of KNORA-E.]{
        \includegraphics[scale=0.325]{content/images/problem_statement/pdf/P1_A.pdf}
        \label{subfig:kne1}
    }
    \hspace*{3cm}
    \subfloat[2nd iteration of KNORA-E.]{
        \includegraphics[scale=0.325]{content/images/problem_statement/pdf/P2_A.pdf}
        \label{subfig:kne2}
    }
    \hspace{10cm}
    \subfloat[3rd iteration of KNORA-E.]{
        \includegraphics[scale=0.325]{content/images/problem_statement/pdf/P3_A.pdf}
        \label{subfig:kne3}
    }
    \hspace*{3cm}
    \subfloat[4th iteration of KNORA-E.]{
        \includegraphics[scale=0.325]{content/images/problem_statement/pdf/P4_A.pdf}
        \label{subfig:kne4}
    }
    \caption{
        KNORA-E iterations when no classifiers 
        correctly classify all samples in the region of competence 
        of the test sample.
        The $\blacktriangle$ is the test sample, 
        the markers {\large$\textcolor{blue}{\circ}$}
        and $\textcolor{red}{\blacksquare}$ are samples from different 
        classes in the region of competence of the test sample,
        and the class of the test sample is "{\large$\textcolor{blue}{\circ}$}".
        (Adapted from \cite{dfp:2017}).
    }
    \label{fig:kne}
\end{center}
\end{figure*}


\begin{comment}
\begin{figure*}[!hbtp]

\begin{center}
    \subfigure[1st iteration of KNORA-E.]{
        \includegraphics[scale=0.325]{content/images/problem_statement/pdf/P1_A.pdf}
        \label{subfig:kne1}
    }
    \hspace*{3cm}
    \subfigure[2nd iteration of KNORA-E.]{
        \includegraphics[scale=0.325]{content/images/problem_statement/pdf/P2_A.pdf}
        \label{subfig:kne2}
    }
    \subfigure[3rd iteration of KNORA-E.]{
        \includegraphics[scale=0.325]{content/images/problem_statement/pdf/P3_A.pdf}
        \label{subfig:kne3}
    }
    \hspace*{3cm}
    \subfigure[4th iteration of KNORA-E.]{
        \includegraphics[scale=0.325]{content/images/problem_statement/pdf/P4_A.pdf}
        \label{subfig:kne4}
    }
    \caption{
        KNORA-E iterations when no classifiers 
        correctly classify all samples in the region of competence 
        of the test sample.
        The $\blacktriangle$ is the test sample, 
        the markers {\large$\textcolor{blue}{\circ}$}
        and $\textcolor{red}{\blacksquare}$ are samples from different 
        classes in the region of competence of the test sample,
        and the class of the test sample is "{\large$\textcolor{blue}{\circ}$}".
        (Adapted from \cite{dfp:2017}).
    }
    \label{fig:kne}
\end{center}
\end{figure*}
\end{comment}

%In the scenario from Figure \ref{fig:kne},
%in the first and second iterations (Figure \ref{subfig:kne1} and \ref{subfig:kne2})
%no classifier correctly classifies all samples in $\Psi$, so, KNORA-E removes
%the sample that is further away from $x_{query}$, respectively, $E$ and $D$, from $\Psi$.
%

In the scenario from Figure \ref{fig:kne},
in the first and second iterations (Figure \ref{subfig:kne1} and \ref{subfig:kne2})
no classifier correctly classifies all samples in $\Psi$. Thus, KNORA-E removes
the samples $E$ and $D$ from $\Psi$, in the first and second iterations, respectively.

In the third iteration (Figure \ref{subfig:kne3}),
again, no classifier correctly classifies all samples in $\Psi$,
then, KNORA-E removes the sample that is further away from $x_{query}$,
$C$, (the last remaining sample of class "$\bluecircle$" in $\Psi$), leaving only two
samples of the class "$\redsquare$" in $\Psi$.
%
In the fourth iteration (Figure \ref{subfig:kne4}), the classifier
$c2$ correctly classifies all samples in $\Psi$ ($A$ and $B$). Thus,
KNORA-E selects $c2$, misclassifying the test sample.
%

This is an issue because when the region of competence of the test
sample has samples from different classes, KNORA-E may change the region
of competence in such a way that it is no longer a good representation
of the local region of the test sample.
% connected
This behavior is not ideal because classifiers that classify all
samples in the region of competence as "$\redsquare$" (such as $c2$)
are selected.
This is a problem especially when dealing with imbalanced dataset,
where a region of competence with samples from the minority class
(class with few samples) can be changed into a region with only
samples from the majority class (class with many samples), even
though the minority class is usually the class of interest.


==> content/chapters/chapter-4/chapter-3-old.tex <==
\newpage
\section{Proposed Algorithms}

\subsection{KNORA DBU}

\subsubsection{Motivation}
For the classification of a test sample $x$, the KNORA U (KNU) selects 
all classifiers that correctly classify at least one of the $K$ 
nearest neighbors of $x$. The KNU sets weights to classifiers, 
proporcional to it's classification rate.

KNU has an issue when the test sample is in an indecision region. It selects
all classifiers that correctly classifies at least one of the $K$ nearest, it
means that it might select classifiers that always classify samples as being
of the same class. When dealing with imbalanced datasets, it might select
classifiers that classify all samples as being of the majority class, which
are not good classifiers for decision regions.

In Figure \ref{fig:knu}, KNU selects all the classifiers, despite
the fact that some classifiers classify all samples as "blue $+$" or
all samples as "red $o$".

\begin{figure}[ht]
\centering
\includegraphics[scale=0.3]{content/images/u/0_U.png}
\caption{Classifiers borders that correctly classify at least 1 of the K nearest neighbors}
\label{fig:knu}
\end{figure}

\subsubsection{Algorithm}

KNORA DB U (KNDBU) selects all classifiers that correctly classify
at least one sample of each class. If no classifiers satisfy this
condition, the KNU is applied.

In Figure \ref{fig:knu}, KNDBU selects only the classifiers
$c2$ and $c3$, leaving behind the classifiers that classify all
samples as the same class ($c1$ and $c4$).


\subsection{KNORA DBE}

\subsubsection{Motivation}
For the classification of a test sample $x$, the KNORA E (KNE) selects 
all classifiers that correctly classify the $K$ nearest neighbors of $x$.
If no classifiers correctly classify all $K$ neighbors, the value of $K$
is decreased, until at least one classifier is selected. If, no classifier
is found, KNE returns all classifiers.

%Figures \ref{subfig:kne1}, \ref{subfig:kne2}, \ref{subfig:kne3} and
%\ref{subfig:kne4} present the iterations of KNE (K=5) over a test sample. 
Figure \ref{fig:kne} presents the iterations of KNE (K=5) over a test sample.
In the first iteration, no classifiers correctly classify all 
K-nearest neighbors, then, the value of K is decreased. The same thing 
happens in the second iteration.

In the last iteration (Figure \ref{subfig:kne3} to \ref{subfig:kne4}),
KNE removes the third nearest sample, leaving
two samples of the same class. This behavior is not ideal because in this
scenario, classifiers that classify all samples as the "blue $+$" class
are selected. When dealing with imbalanced dataset, classifiers that
classify all samples as the majority class will be selected, instead of
classifiers that have decision boundaries in that region.

\subsubsection{Algorithm}

In the KNORA DBE (KNDBE), if no classifiers correctly classify all $K$ 
neighbors of $x$, the value of $K$ is decreased but maintaining the indecision 
region, that means that KNDBE removes the further neighbor only if the 
remaining neighbors belong to different classes, otherwise, the second 
further neighbor is removed (and so on).

%Figures \ref{subfig:kndbe1}, \ref{subfig:kndbe2}, \ref{subfig:kndbe3},
%\ref{subfig:kndbe4} present the iterations of KNDBE (K=5).
Figure \ref{fig:kndbe} presents the iterations of KNDBE (K=5).
The first two iterations are the same for KNE and KNDBE. In the last iteration
(Figure \ref{subfig:kndbe3} to \ref{subfig:kndbe4}) the KNDBE removes the second further neighbor
instead of the further in order to maintain the same set of classes of the original neighborhood.
This makes the algorithm to select only classifiers that correctly classify all samples in an
heterogeneous neighborhood.

When dealing with imbalanced datasets, classifiers that classify all samples
as the majority class will never be selected, unless no classifiers satisfy the
KNDBE criteria.

\input{content/chapters/chapter-3/fig.tex}



==> content/chapters/chapter-4/fig.tex <==



==> content/chapters/chapter-4/pseudocode.tex <==
\begin{algorithm}[H]
%\begin{algorithm*}
%\begin{figure*}
\caption{ABag}
\begin{algorithmic}[1]
	\REQUIRE $\mathcal{T}$: training set.
	\REQUIRE $\mathcal{V}$: validation set.
    \REQUIRE $N$: size of the pool.
    \REQUIRE $K$: number of classifiers to be added in each iteration.
    \REQUIRE $\alpha$: fitness parameter.
    \REQUIRE \textit{diversity}: diversity metric to be used.
    \STATE $\mathcal{P} \gets$ empty list of classifiers.
	\STATE Generate classifier using a random bootstrap of samples and add it to $\mathcal{P}$.
    \WHILE {$|\mathcal{P}| < N$}
        \STATE \textit{weights} $\gets$ $Probability_{class_i} = 1 - \dfrac{FN_{class_i}}{\sum\nolimits_{class_j \in classes} FN_{class_j}}$.
        \STATE $C$ = $K$ classifiers using \textit{weights} to perform the bootstrap of samples.
        \FORALL {classifier $c_i \in C$}
            \STATE Add $c_i$ to $\mathcal{P}$.
            \STATE \textit{acc} $\gets AUC(\mathcal{P})$
            \STATE \textit{div} $\gets \text{\textit{diversity}}(\mathcal{P})$
            \STATE $fitness(c_i) \gets \alpha \times acc + (1 - \alpha) \times div$
            \STATE Remove $c_i$ from $\mathcal{P}$.
		\ENDFOR
        \STATE $best \gets argmax(fitness, C)$
        \STATE Add $C[best]$ to $\mathcal{P}$
        \STATE Update \textit{weights}
	\ENDWHILE
	\RETURN $\mathcal{P}$
\end{algorithmic}
\label{alg:abag}
%\end{figure*}
%\end{algorithm*}
\end{algorithm}




==> content/chapters/chapter-5/auc-table.tex <==
% !TEX encoding = ISO88591

\begin{table*}[htbp]
\center
\caption{Average, standard deviation AUC, and Wilcoxon Signed Rank Test.}
\begin{tabular}{lcccccccccc}

\hline
\multicolumn{1}{c}{Dataset} & \multicolumn{ 2}{c}{ICS-Bagging-40} & \multicolumn{ 2}{c}{SICS-Bagging-40} & \multicolumn{ 2}{c}{SMOTEBagging-40} & \multicolumn{ 2}{c}{Bagging-40} & \multicolumn{ 2}{c}{RandomSubspace-40} \\ 
\hline
\hline
glass1 & \textbf{0.7923} & \textbf{0.0500} & 0.7829 & 0.0193 & 0.7816 & 0.0770 & 0.7521 & 0.0529 & 0.5133 & 0.0267 \\ 
pima & \textbf{0.7390} & \textbf{0.0194} & 0.7377 & 0.0189 & 0.6988 & 0.0307 & 0.7215 & 0.0227 & 0.5766 & 0.0345 \\ 
iris0 & \textbf{1.0000} & \textbf{0.0000} & \textbf{1.0000} & \textbf{0.0000} & \textbf{1.0000} & \textbf{0.0000} & \textbf{1.0000} & \textbf{0.0000} & 0.9700 & 0.0600 \\ 
yeast1 & 0.7309 & 0.0343 & 0.7204 & 0.0237 & \textbf{0.7314} & \textbf{0.0282} & 0.6810 & 0.0187 & 0.5288 & 0.0342 \\ 
vehicle2 & 0.9592 & 0.0168 & 0.9630 & 0.0159 & \textbf{0.9669} & \textbf{0.0127} & 0.9594 & 0.0225 & 0.5596 & 0.0403 \\ 
vehicle3 & 0.7368 & 0.0188 & \textbf{0.7566} & \textbf{0.0162} & 0.7300 & 0.0083 & 0.6600 & 0.0226 & 0.5008 & 0.0106 \\ 
ecoli1 & 0.8722 & 0.0497 & \textbf{0.8795} & \textbf{0.0444} & 0.8642 & 0.0414 & 0.8480 & 0.0454 & 0.5086 & 0.0172 \\ 
ecoli2 & 0.8855 & 0.0495 & \textbf{0.8861} & \textbf{0.0439} & 0.8670 & 0.0529 & 0.8714 & 0.0464 & 0.5000 & 0.0000 \\ 
glass6 & 0.8917 & 0.0190 & \textbf{0.8965} & \textbf{0.0643} & 0.8886 & 0.0361 & 0.8865 & 0.0624 & 0.7440 & 0.1694 \\ 
yeast3 & \textbf{0.9089} & \textbf{0.0273} & 0.9045 & 0.0248 & 0.9055 & 0.0095 & 0.8434 & 0.0337 & 0.5000 & 0.0000 \\ 
ecoli3 & 0.8047 & 0.0967 & \textbf{0.8223} & \textbf{0.0590} & 0.7525 & 0.0827 & 0.7724 & 0.0677 & 0.5000 & 0.0000 \\ 
vowel0 & 0.9483 & 0.0573 & 0.9594 & 0.0546 & 0.9455 & 0.0547 & 0.9589 & 0.0540 & 0.4994 & 0.0011 \\ 
glass4 & 0.8750 & 0.1877 & \textbf{0.8825} & \textbf{0.1915} & 0.8708 & 0.0982 & 0.7467 & 0.1654 & 0.5000 & 0.0000 \\ 
ecoli4 & 0.8405 & 0.1143 & \textbf{0.8655} & \textbf{0.0721} & 0.8155 & 0.1194 & 0.8671 & 0.1326 & 0.5000 & 0.0000 \\ 
page-blocks-1-3\_vs\_4 & \textbf{0.9978} & \textbf{0.0045} & \textbf{0.9978} & \textbf{0.0045} & \textbf{0.9978} & \textbf{0.0045} & 0.9766 & 0.0414 & 0.6378 & 0.0612 \\ 
\hline
Average & 0.8655 & 0.0497 & \textbf{0.8703} & \textbf{0.0435} & 0.8544 & 0.0438 & 0.8363 & 0.0526 & 0.5693 & 0.0303 \\ 
\hline
P-value (ICS-Bagging) & \multicolumn{ 2}{c}{NA} & \multicolumn{ 2}{c}{0.9420743} & \multicolumn{ 2}{c}{0.004387317} & \multicolumn{ 2}{c}{0.005503956} & \multicolumn{ 2}{c}{0.0003274792} \\ 
Result (ICS-Bagging) & \multicolumn{ 2}{c}{NA} & \multicolumn{ 2}{c}{$-$} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{$+$} \\ 
P-value (SICS-Bagging) & \multicolumn{ 2}{c}{0.05792575} & \multicolumn{ 2}{c}{NA} & \multicolumn{ 2}{c}{0.005373392} & \multicolumn{ 2}{c}{0.0007616379} & \multicolumn{ 2}{c}{0.0003274792} \\ 
result (SICS-Bagging) & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{NA} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{$+$} \\ 
\hline
\end{tabular}
\label{tab:auc_40}
\end{table*}


==> content/chapters/chapter-5/datasets-table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                                  %%
%%  This is a LaTeX2e table fragment exported from Gnumeric.        %%
%%                                                                  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[H]
\centering
\begin{tabular}{cllll}
\hline
\textbf{Label}	&\textbf{Dataset}	&\textbf{Atribute}	& \textbf{Instances}	&\textbf{IR}	\\
\hline \hline
1	&pima			&8 (8/0/0)	    &768		&1.87	\\
2	&yeast1			&8 (8/0/0)	    &1484		&2.46	\\
3	&vehicle2		&18 (0/18/0)	&846		&2.88	\\
4	&vehicle1		&18 (0/18/0)	&846		&2.9	\\
5	&vehicle3		&18 (0/18/0)	&846		&2.99	\\
6	&vehicle0		&18 (0/18/0)	&846		&3.25	\\
7	&ecoli2			&7 (7/0/0)	    &336		&5.46	\\
8	&segment0		&19 (19/0/0)	&2308		&6.02	\\
9	&ecoli3			&7 (7/0/0)	    &336		&8.6	\\
10	&yeast05679vs4	&8 (8/0/0)	    &528		&9.35	\\
11	&vowel0			&13 (10/3/0)	&988		&9.98	\\
12	&glass016vs2	&9 (9/0/0)	    &192		&10.29	\\
13	&glass2			&9 (9/0/0)	    &214		&11.59	\\
14	&shuttlec0vsc4	&9 (0/9/0)	    &1829		&13.87	\\
15	&yeast1vs7	    &7 (7/0/0)		&459		&14.3	\\
\hline
\end{tabular}
\caption{Datasets used in the experiment}
\label{tab:datasets}
\end{table}


==> content/chapters/chapter-5/div-table.tex <==
% !TEX encoding = ISO88591

\begin{table*}[ht]
\center
\caption{Average, standard deviation Entropy Measure $e$, and Wilcoxon Signed Rank Test.}
\begin{tabular}{lcccccccccc}
\hline
\multicolumn{1}{c}{Dataset} & \multicolumn{ 2}{c}{ICS-Bagging-40} & \multicolumn{ 2}{c}{SICS-Bagging-40} & \multicolumn{ 2}{c}{SMOTEBagging-40} & \multicolumn{ 2}{c}{Bagging-40} & \multicolumn{ 2}{c}{RandomSubspace-40} \\ 
\hline
\hline
glass1 & 0.4445 & 0.0560 & 0.4314 & 0.0570 & 0.4177 & 0.0464 & 0.3786 & 0.0531 & \textbf{0.5242} & \textbf{0.0212} \\ 
pima & 0.4284 & 0.0133 & 0.4130 & 0.0197 & \textbf{0.4303} & \textbf{0.0174} & 0.4131 & 0.0196 & 0.0080 & 0.0041 \\ 
iris0 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & \textbf{0.3866} & \textbf{0.0067} \\ 
yeast1 & \textbf{0.4342} & \textbf{0.0230} & 0.3926 & 0.0256 & 0.3779 & 0.0200 & 0.3410 & 0.0029 & 0.1502 & 0.0163 \\ 
vehicle2 & 0.1006 & 0.0148 & 0.0809 & 0.0039 & 0.0849 & 0.0059 & 0.0886 & 0.0126 & \textbf{0.3900} & \textbf{0.0352} \\ 
vehicle3 & \textbf{0.3900} & \textbf{0.0219} & 0.3774 & 0.0248 & 0.3757 & 0.0239 & 0.3661 & 0.0177 & 0.3431 & 0.0296 \\ 
ecoli1 & 0.1542 & 0.0361 & 0.1555 & 0.0479 & 0.1474 & 0.0340 & 0.1456 & 0.0337 & \textbf{0.2441} & \textbf{0.0156} \\ 
ecoli2 & \textbf{0.1556} & \textbf{0.0440} & 0.1377 & 0.0347 & 0.1174 & 0.0203 & 0.1216 & 0.0286 & 0.1189 & 0.0189 \\ 
glass6 & 0.1108 & 0.0550 & 0.0894 & 0.0235 & 0.0708 & 0.0305 & 0.0613 & 0.0148 & \textbf{0.1592} & \textbf{0.0158} \\ 
yeast3 & 0.0767 & 0.0076 & 0.0717 & 0.0110 & 0.0619 & 0.0086 & 0.0825 & 0.0086 & \textbf{0.1842} & \textbf{0.0260} \\ 
ecoli3 & 0.1187 & 0.0364 & 0.1200 & 0.0339 & 0.1089 & 0.0361 & \textbf{0.1246} & \textbf{0.0290} & 0.0844 & 0.0066 \\ 
vowel0 & 0.0346 & 0.0176 & 0.0309 & 0.0148 & 0.0237 & 0.0084 & 0.0299 & 0.0069 & \textbf{0.1123} & \textbf{0.0449} \\ 
glass4 & 0.0684 & 0.0299 & 0.0623 & 0.0288 & 0.0557 & 0.0289 & 0.0944 & 0.0312 & \textbf{0.1087} & \textbf{0.0341} \\ 
ecoli4 & 0.0460 & 0.0228 & \textbf{0.0476} & \textbf{0.0049} & 0.0253 & 0.0125 & 0.0333 & 0.0151 & 0.0461 & 0.0081 \\ 
page-blocks-1-3\_vs\_4 & 0.0052 & 0.0065 & 0.0020 & 0.0035 & 0.0012 & 0.0013 & 0.0269 & 0.0090 & \textbf{0.0484} & \textbf{0.0088} \\ 
\hline
\multicolumn{1}{c}{Average} & 0.1712 & 0.0257 & 0.1608 & 0.0223 & 0.1533 & 0.0196 & 0.1538 & 0.0189 & \textbf{0.1939} & \textbf{0.0195} \\ 
\hline
\multicolumn{1}{c}{P-value (ICS-Bagging)} & \multicolumn{ 2}{c}{NA} & \multicolumn{ 2}{c}{0.001078881} & \multicolumn{ 2}{c}{0.0006125118} & \multicolumn{ 2}{c}{0.03201965} & \multicolumn{ 2}{c}{0.9990406} \\ 
\multicolumn{1}{c}{Result (ICS-Bagging)} & \multicolumn{ 2}{c}{NA} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{$-$} \\ 
\multicolumn{1}{c}{P-value (SICS-Bagging)} & \multicolumn{ 2}{c}{0.9982489} & \multicolumn{ 2}{c}{NA} & \multicolumn{ 2}{c}{0.007826775} & \multicolumn{ 2}{c}{0.1501449} & \multicolumn{ 2}{c}{0.9042768} \\ 
\multicolumn{1}{c}{Result (SICS-Bagging)} & \multicolumn{ 2}{c}{$-$} & \multicolumn{ 2}{c}{NA} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{$=$} & \multicolumn{ 2}{c}{$-$} \\ 
\hline
\end{tabular}
\label{tab:div_40}
\end{table*}



==> content/chapters/chapter-5/sts.chapter-5.tex <==
\section{Experiments}
\label{sec:experiments}

We evaluated KNORA-B and KNORA-BI using 40 datasets as proposed
in \cite{dfp:2017}. The datasets were taken from the imbalanced datasets
module in the Knowledge Experiments based on Evolutionary Learning (KEEL)
repository \cite{keel}.
Table \ref{tab:datasets} presents the details about the datasets
used in our experiments: label, name, number of features,
number of samples, and imbalance ratio (IR).

\begin{table}[htbp]
\begin{center}
\caption{Summary of the 40 datasets used in the experiments: label, name, number of features, number of samples, and imbalance ratio (from \cite{dfp:2017}).}
\label{tab:datasets}
\resizebox{0.450\textwidth}{!}{
\footnotesize
    \begin{tabular}{clrrr}
        \hline
        
Label & Name            & \#Feats. & \#Samples & IR \\
        \hline
        \hline
1     & glass1          & 9     & 214        & 1.82 \\
2     & ecoli0vs1       & 7     & 220        & 1.86 \\
3     & wisconsin       & 9     & 683        & 1.86 \\
4     & pima            & 8     & 768        & 1.87 \\ 
5     & iris0           & 4     & 150        & 2.00 \\
6     & glass0          & 9     & 214        & 2.06 \\
7     & yeast1          & 8     & 1484       & 2.46 \\ 
8     & vehicle2        & 18    & 846        & 2.88 \\ 
9     & vehicle1        & 18    & 846        & 2.9  \\
10    & vehicle3        & 18    & 846        & 2.99 \\ 
11    & glass0123vs456  & 9     & 214        & 3.2  \\ 
12    & vehicle0        & 18    & 846        & 3.25 \\ 
13    & ecoli1          & 7     & 336        & 3.36 \\ 
14    & new-thyroid1    & 5     & 215        & 5.14 \\ 
15    & new-thyroid2    & 5     & 215        & 5.14 \\
16    & ecoli2          & 7     & 336        & 5.46 \\
17    & segment0        & 19    & 2308       & 6.00 \\
18    & glass6          & 9     & 214        & 6.38 \\
19    & yeast3          & 8     & 1484       & 8.10 \\
20    & ecoli3          & 7     & 336        & 8.60 \\ 
21    & yeast-2vs4      & 8     & 514        & 9.08 \\
22    & yeast-05679vs4  & 8     & 528        & 9.35 \\
23    & vowel0          & 13    & 988        & 9.98 \\
24    & glass-016vs2    & 9     & 192        & 10.29 \\
25    & glass2          & 9     & 214        & 11.59 \\
26    & shuttle-c0vsc4  & 9     & 1829       & 13.87 \\
27    & yeast-1vs7      & 7     & 459        & 14.30 \\
28    & glass4          & 9     & 214        & 15.47 \\
29    & ecoli4          & 7     & 336        & 15.80 \\
30    & page-blocks-13vs4   & 10& 472        & 15.86 \\
31    & glass-0-1-6\_vs\_5  & 9 & 184        & 19.44 \\
32    & shuttle-c2-vs-c4    & 9 & 129        & 20.50 \\
33    & yeast-1458vs7   & 8     & 693        & 22.10 \\
34    & glass5          & 9     & 214        & 22.78 \\
35    & yeast-2vs8      & 8     & 482        & 23.10 \\
36    & yeast4          & 8     & 1484       & 28.10 \\
37    & yeast-1289vs7   & 8     & 947        & 30.57 \\
38    & yeast5          & 8     & 1484       & 32.73 \\
39    & ecoli-0137vs26  & 7     & 281        & 39.14 \\
40    & yeast6          & 8     & 1484       & 41.40 \\
        \hline
\end{tabular}
}%resizebox
\end{center}
\end{table}

For each dataset, the data was partitioned using the
\textit{stratified 5-fold cross-validation}
(1 fold used for testing, and 4 folds for validation/training)
followed by a
\textit{stratified 4-fold cross-validation}
(the 4 folds in validation/training divided in 1 for
validation, and 3 for training), resulting in 20
replications for each dataset using 20\% for testing,
20\% for validation, and 60\% for training.

The analysis is conducted using 8 DES techniques from the
literature, their respective FIRE-DES versions (using the F prefix), and
3 state-of-the-art DES techniques.
Table \ref{tab:dsexp} shows the dynamic selection techniques
used in our experiments, their categories and references.
Following the approach using in \cite{dfp:2017},
we use a pool of classifiers composed of 100 Perceptrons
generated using the Bootstrap AGGregatING (Bagging) technique \cite{bagging:1996},
and a region of competence size $K = 7$.

\begin{table}[h]
\begin{center}
\caption{
    Dynamic selection techniques considered in the experiments (From \cite{dfp:2017}).
}
\label{tab:dsexp}
\resizebox{0.450\textwidth}{!}{
\begin{tabular}{lll}
\hline
Technique & Category & Reference \\
\hline
\hline
\textbf{DES} & &  \\
Overall Local Accuracy (OLA)        & Accuracy      & Woods et al. \cite{dcs_la:1996} \\
Local Class Accuracy (LCA)          & Accuracy      & Woods et al. \cite{dcs_la:1996} \\
A Priori (APri)                     & Probabilistic &  Giacinto et al. \cite{dcs_la:1999} \\
A Posteriori (APos)                 & Probabilistic &  Giacinto et al. \cite{dcs_la:1999} \\
Multiple Classifier Behavior (MCB)  & Behavior      & Giacinto et al. \cite{mcb:2001} \\
Dynamic Selection KNN (DSKNN)       & Diversity     & Santana et al. \cite{dsknn:2006} \\
K-Nearests Oracles Union (KNORA-U)      & Oracle        & Ko et al. \cite{des:2008} \\
K-Nearests Oracles Eliminate (KNORA-E)  & Oracle        & Ko et al. \cite{des:2008} \\
\textbf{State-of-the-art} & & \\
Randomized Reference Classifier (RRC)   & Probabilistic &   Woloszynski et al. \cite{rrc:2011}      \\
META-DES                                & Meta-learning &   Cruz et al. \cite{metades:2015}         \\
META-DES.Oracle                         & Meta-learning &   Cruz et al. \cite{metadesoracle:2017}   \\
\hline
\end{tabular}}
\end{center}
\end{table}

Following the approach in \cite{dfp:2017}, 
we used the Area Under the ROC Curve (AUC) \cite{auc:1997}
for performance evaluation since
it is a suitable  metric for binary imbalanced
datasets \cite{cip:2013} \cite{dfp:2017}.
We also used the Wilcoxon Signed Rank Test \cite{wilcox:2016} \cite{wilcoxon:1945}
and the Sign Test \cite{signedtest:2006} to perform a pairwise comparison of the
proposed techniques with the techniques from the literature.

\subsection{Results}

Table \ref{tab:results} presents the overall results.
For each technique, the table shows:
the mean AUC and standard deviation,
the average ranking,
and the \textit{p-value} and result of the Wilcoxon Signed Rank Test
comparing KNORA-B and KNORA-BI with the DES technique
($+$/$=$/$-$ signs mean the proposed technique had statistically
better, equal, and worse classification performance
considering a confidence level $\alpha = 0.05$).

\begin{table}[h]
%\footnotesize
\begin{center}
\caption{
    Overall results.
}
\label{tab:results}
\resizebox{0.495\textwidth}{!}{
\begin{tabular}{lrrlrlr}
\hline
DES &              AUC &   RANK &      \multicolumn{2}{c}{KNORA-B (\textit{p-value})} &      \multicolumn{2}{c}{KNORA-BI (\textit{p-value})}  \\
\hline
\hline
            KNORA-B &  0.7989 (0.0721) &  11.28 &             \multicolumn{2}{c}{$NA$} &  $5.60 \times e^{-6}$ &           $+$ \\
           KNORA-BI &  \textbf{0.8136 (0.0743)} &         \textbf{6.80} &                0.9999 &          $-$ &  \multicolumn{2}{c}{$NA$} \\
            OLA &  0.7911 (0.0709) &  13.60 &                0.0623 &          $=$ &  $1.40 \times e^{-7}$ &           $+$ \\
            LCA &  0.7809 (0.0737) &  13.30 &                0.0332 &          $+$ &  $7.20 \times e^{-6}$ &           $+$ \\
           APRI &  0.7537 (0.0628) &  16.38 &  $3.20 \times e^{-5}$ &          $+$ &  $9.80 \times e^{-7}$ &           $+$ \\
           APOS &  0.7380 (0.0658) &  18.01 &  $1.10 \times e^{-5}$ &          $+$ &  $4.70 \times e^{-7}$ &           $+$ \\
            MCB &  0.7443 (0.0566) &  17.32 &  $2.10 \times e^{-6}$ &          $+$ &  $6.40 \times e^{-7}$ &           $+$ \\
          DSKNN &  0.7728 (0.0602) &  13.32 &                0.0107 &          $+$ &  $6.10 \times e^{-5}$ &           $+$ \\
            KNORA-U &  0.7560 (0.0548) &  15.39 &                0.0002 &          $+$ &  $6.80 \times e^{-6}$ &           $+$ \\
            KNORA-E &  0.8003 (0.0703) &  10.66 &                0.8298 &          $=$ &                0.0002 &           $+$ \\
          FKNORA-BI &  0.8083 (0.0758) &   9.01 &                0.9976 &          $-$ &                0.0003 &           $+$ \\
           FKNORA-B &  0.8042 (0.0772) &  10.34 &                0.9860 &          $-$ &                0.0001 &           $+$ \\
           FOLA &  0.8017 (0.0767) &  12.97 &                0.5026 &          $=$ &  $3.80 \times e^{-6}$ &           $+$ \\
           FLCA &  0.7946 (0.0777) &  11.84 &                0.5554 &          $=$ &  $8.30 \times e^{-6}$ &           $+$ \\
          FAPRI &  0.7930 (0.0802) &  13.10 &                0.1940 &          $=$ &  $1.60 \times e^{-6}$ &           $+$ \\
          FAPOS &  0.7681 (0.0809) &  15.86 &                0.0001 &          $+$ &  $1.40 \times e^{-7}$ &           $+$ \\
           FMCB &  0.8058 (0.0760) &   8.80 &                0.9235 &          $=$ &                0.0921 &           $=$ \\
         FDSKNN &  0.8006 (0.0767) &  11.43 &                0.5250 &          $=$ &  $2.00 \times e^{-6}$ &           $+$ \\
           FKNORA-U &  0.8081 (0.0765) &   8.38 &                0.9712 &          $-$ &                0.1009 &           $=$ \\
           FKNORA-E &  0.8055 (0.0768) &   9.59 &                0.9962 &          $-$ &                0.0002 &           $+$ \\
           META &  0.8100 (0.0635) &   8.20 &                0.9742 &          $-$ &                0.4362 &           $=$ \\
         META.O &  0.8067 (0.0649) &   8.16 &                0.9509 &          $-$ &                0.3454 &           $=$ \\
            RRC &  0.7934 (0.0658) &  12.26 &                0.1805 &          $=$ &                0.0057 &           $+$ \\
\hline
\end{tabular}}
\end{center}
\end{table}


Table \ref{tab:results} show that KNORA-BI achieved the highest
mean AUC ($0.8136$) and the best average ranking ($6.80$), outperforming all techniques considered in this work.
Moreover, it statistically outperformed 18 out of 22 techniques according to the Wilcoxon Signed Rank test.
%being statistically equivalent to META, META.O, and FKNORA-U.
Table \ref{tab:results} also shows that KNORA-B was not as good as KNORA-BI,
achieving the 12th best AUC ($0.7989$), and being statistically equivalent to KNORA-E ($0.8003$). However,
it was only statistically outperformed by 7 out of 22 techniques, where 3 of those are
variations of the techniques proposed in this paper (KNORA-BI, FKNORA-B, and FKNORA-BI).

In addition, FKNORA-B ($0.8042$) outperformed KNORA-B ($0.7989$) with statistical confidence,
meaning FIRE-DES caused a significant increase in classification performance in KNORA-B.
This increase in AUC is explained in the scenario that no classifier was selected
and the region of competence has only one sample from each class remaining.
In this scenario, KNORA-B applies KNORA-E on the entire pool of classifiers
while FKNORA-B applies KNORA-E on the set of pre-selected classifiers
(avoiding the selection of incompetent classifiers that classify all samples
in the region of competence as being from the same class).

On the other hand, KNORA-BI ($0.8136$) outperformed FKNORA-BI ($0.8083$) with statistical confidence,
meaning FIRE-DES caused a significant decrease in classification performance in KNORA-BI.
KNORA-BI allows the region of competence to be reduced until there is
only minority class samples, allowing to the selection of classifiers that classify all samples in
the region of competence as minority class samples, while FKNORA-BI does not allow the selection of
such classifiers. Because the minority class is so rare, preventing a DES technique
from selecting a classifier that classifies all samples in the region of competence as minority
class sample is not advantageous, specially because correctly classifying 1 minority class sample
has a higher impact than misclassifying 1 majority class sample,
which explains why KNORA-BI was better without FIRE-DES.

%We also conducted a pairwise comparison using the Sign Test \cite{signedtest:2006},
%calculated using the wins, ties, and losses achieved by the KNORA-B and KNORA-BI when compared
%to the other DS techniques considered in the experiments. Figures \ref{fig:wtl_knb_all} and \ref{fig:wtl_knbi_all} present
%the results of the Sign test for the KNORA-B and KNORA-BI respectively.
Figures \ref{fig:wtl_knb_all} and \ref{fig:wtl_knbi_all}
present pairwise comparisons of, respectively, KNORA-B with
other techniques and KNORA-BI with other techniques
The comparisons use the Sign Test \cite{signedtest:2006},
calculated using the wins, ties, and losses of
KNORA-B and other techniques (Figure \ref{fig:wtl_knb_all})
and KNORA-BI and other techniques (Figure \ref{fig:wtl_knbi_all}).

\begin{figure}[h]
\centering
\includegraphics[width=2.5in, height=4.2in]{content/images/results/WTL_KNB_ALL.pdf}
\caption{
    Classification performance comparison of KNORA-B with different DES techniques
    in terms of wins, ties and losses considering the average AUC in the 40 datasets.
    The dashed lines (left to right) illustrates the critical values
    $n_c = \{24.05, 25.20, 27.37\}$ considering significance levels of
    $\alpha = \{0.10, 0.05, 0.01\}$, respectively.
}
\label{fig:wtl_knb_all}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=2.5in, height=4.2in]{content/images/results/WTL_KNBI_ALL.pdf}
\caption{
    Classification performance comparison of KNORA-BI with different DES techniques
    in terms of wins, ties and losses considering the average AUC in the 40 datasets.
    The dashed lines (left to right) illustrates the critical values
    $n_c = \{24.05, 25.20, 27.37\}$ considering significance levels of
    $\alpha = \{0.10, 0.05, 0.01\}$, respectively.
}
\label{fig:wtl_knbi_all}
\end{figure}

For a comparison between one of the proposed techniques and a technique T,
the null hypothesis $H_0$ was that the proposed technique is not statistically different than T,
%the proposed technique is not statistically different the techniques from the literatue,
and a rejection of $H_0$ meant that the proposed technique is statistically better than T.
$H_0$ is rejected if the number of wins plus half of the number of ties
is greater or equal to $n_c$ (Equation \ref{eq:ncp_knb}):

\begin{equation}
    \label{eq:ncp_knb}
    n_c = \dfrac{n_{exp}}{2} + z_{\alpha} \times \dfrac{\sqrt[2]{n_{exp}}}{2}
\end{equation}

\noindent where $n_{exp} = 40$ (the number of experiments),
$n_c = \{24.05, 25.20, 27.37\}$, respectively for the levels of signficance
$\alpha = \{0.10, 0.05, 0.01\}$.

Figure \ref{fig:wtl_knb_all} shows that, considering $\alpha = 0.05$,
KNORA-B statistically outperformed 7 out of the 8 regular DES techniques,
being only statistically equivalent to KNORA-E.
Comparing with FIRE-DES framework, KNORA-B outperformed only FAPOS (the worst of FIRE-DES in our experiments).
KNORA-B was not better than any of the state-of-art DES techniques.

Figure \ref{fig:wtl_knbi_all} shows that overall KNORA-BI statistically outperformed
a signficant number of techniques (18 out of 22), even for level of significance
$\alpha = 0.01$ (14 out of 22).
Considering a $\alpha = 0.05$, KNORA-BI outperformed the variations of the
proposed techniques (KNORA-B, FKNORA-B, and FKNORA-BI),
all regular DES techniques from the literature, and most of FIRE-DES techniques
(not outperforming only FKNORA-U and FMCB), and state-of-art DES technique RRC.

%KNORA-B and KNORA-E had statistically equivalent classification performance,
%even though KNORA-B tackles a KNORA-E issue.

\begin{figure}[h]
\centering
\includegraphics[scale=0.45]{content/images/results/KNB_KNBI_IR.pdf}
\caption{AUC difference between KNORA-B and KNORA-E, and between KNORA-BI and KNORA-E.}
\label{fig:knbir}
\end{figure}

Figure \ref{fig:knbir} presents the average AUC difference from KNORA-B and KNORA-BI to
KNORA-E considering the datasets 1-10, 11-20, 21-30, and 31-40.
This figure shows that KNORA-B is better than KNORA-E optimally in 21-30
and slightly better in 31-40, while KNORA-BI was always better than KNORA-E
(the more the imbalance ratio the higher the difference).
This confirms that for all imbalance levels KNORA-BI was better than KNORA-E,
while KNORA-B was only better than KNORA-B for high imbalance level.


Based on the results, we can state with confidence
that KNORA-B achieved statistically equivalent performance of KNORA-E,
and KNORA-BI statistically outperformed KNORA-E and all other techniques
considered in this experiment.





==> content/chapters/chapter-5/table.tex <==

\begin{table}[htbp]
\centering
\caption{Average AUC}
\begin{tabular}{lcccccc}
\hline
Datasets & KNDBE & KNDBU & KNE & KNU & OLA & LCA \\ 
\hline
\hline
glass1 & 0.7388 & \textbf{0.7425} & 0.7388 & 0.7388 & 0.7120 & 0.7106 \\ 
ecoli-0\_vs\_1 & \textbf{0.9667} & 0.9537 & \textbf{0.9667} & \textbf{0.9667} & 0.9566 & 0.9207 \\ 
wisconsin & 0.9594 & \textbf{0.9635} & 0.9594 & 0.9561 & 0.9529 & 0.9447 \\ 
pima & 0.6589 & 0.6693 & 0.6644 & \textbf{0.6737} & 0.6537 & 0.6502 \\ 
iris0 & 1.0000 & \textbf{1.0000} & \textbf{1.0000} & \textbf{1.0000} & \textbf{1.0000} & \textbf{1.0000} \\ 
glass0 & 0.7847 & \textbf{0.7995} & 0.7776 & 0.7780 & 0.7635 & 0.7707 \\ 
yeast1 & 0.6410 & \textbf{0.6604} & 0.6393 & 0.6553 & 0.6390 & 0.6358 \\ 
vehicle2 & 0.9347 & 0.9337 & 0.9347 & \textbf{0.9350} & 0.9168 & 0.9015 \\ 
vehicle1 & 0.6159 & \textbf{0.6514} & 0.6151 & 0.6367 & 0.6246 & 0.6116 \\ 
vehicle3 & 0.6658 & \textbf{0.6950} & 0.6674 & 0.6775 & 0.6730 & 0.6558 \\ 
glass-0-1-2-3\_vs\_4-5-6 & 0.8291 & \textbf{0.8631} & 0.8291 & 0.8251 & 0.8174 & 0.8234 \\ 
vehicle0 & 0.8875 & 0.9079 & 0.8850 & \textbf{0.9104} & 0.8712 & 0.8638 \\ 
ecoli1 & 0.8851 & 0.8836 & 0.8765 & \textbf{0.8913} & 0.8552 & 0.8486 \\ 
new-thyroid1 & 0.9230 & \textbf{0.9544} & 0.9230 & 0.9258 & 0.8687 & 0.8659 \\ 
new-thyroid2 & 0.8802 & \textbf{0.9317} & 0.8802 & 0.8944 & 0.8829 & 0.8829 \\ 
ecoli2 & 0.8888 & \textbf{0.9326} & 0.8888 & 0.9278 & 0.9035 & 0.9108 \\ 
segment0 & 0.9889 & \textbf{0.9891} & 0.9889 & 0.9874 & 0.9856 & 0.9851 \\ 
glass6 & 0.8325 & 0.8271 & 0.8325 & 0.8325 & \textbf{0.8352} & 0.8325 \\ 
yeast3 & 0.8349 & 0.8425 & 0.8349 & 0.8341 & 0.8353 & \textbf{0.8440} \\ 
ecoli3 & 0.7515 & 0.7827 & 0.7658 & \textbf{0.7910} & 0.7212 & 0.7036 \\ 
yeast-2\_vs\_4 & 0.7911 & 0.8310 & 0.7911 & \textbf{0.8353} & 0.7947 & 0.7867 \\ 
yeast-0-5-6-7-9\_vs\_4 & 0.6738 & \textbf{0.6955} & 0.6738 & 0.6667 & 0.6757 & 0.6459 \\ 
vowel0 & 0.9661 & \textbf{0.9694} & 0.9661 & 0.9661 & 0.9383 & 0.9150 \\ 
glass-0-1-6\_vs\_2 & \textbf{0.5995} & 0.5938 & \textbf{0.5995} & 0.5555 & 0.5326 & 0.5440 \\ 
glass2 & 0.4795 & 0.4593 & 0.4795 & 0.4923 & \textbf{0.5077} & 0.4718 \\ 
shuttle-c0-vs-c4 & \textbf{0.9960} & \textbf{0.9960} & \textbf{0.9960} & \textbf{0.9960} & \textbf{0.9960} & \textbf{0.9960} \\ 
yeast-1\_vs\_7 & 0.5442 & \textbf{0.6399} & 0.5442 & 0.5442 & 0.5360 & 0.6205 \\ 
glass4 & 0.7350 & 0.7585 & 0.7350 & 0.7301 & 0.7326 & \textbf{0.7942} \\ 
ecoli4 & \textbf{0.8984} & 0.8468 & \textbf{0.8984} & 0.8500 & 0.8734 & 0.8734 \\ 
page-blocks-1-3\_vs\_4 & \textbf{0.9633} & 0.9388 & \textbf{0.9633} & 0.9433 & 0.8500 & 0.8322 \\ 
glass-0-1-6\_vs\_5 & 0.7414 & \textbf{0.7886} & 0.7414 & 0.6943 & 0.6943 & 0.6943 \\ 
yeast-1-4-5-8\_vs\_7 & 0.4962 & \textbf{0.5827} & 0.4970 & 0.4962 & 0.5023 & 0.4993 \\ 
yeast-2\_vs\_8 & 0.7489 & \textbf{0.7696} & 0.7489 & 0.7489 & 0.7489 & 0.7478 \\ 
yeast4 & 0.5939 & 0.6183 & 0.6039 & 0.5753 & \textbf{0.6219} & 0.5789 \\ 
yeast-1-2-8-9\_vs\_7 & 0.4973 & 0.4864 & 0.4978 & 0.4995 & 0.5069 & \textbf{0.5380} \\ 
yeast5 & 0.7931 & 0.8351 & \textbf{0.8045} & 0.8017 & 0.7556 & 0.7434 \\ 
yeast6 & 0.7095 & 0.7764 & 0.7095 & 0.7370 & \textbf{0.7489} & 0.7774 \\ 
\hline
Average & 0.7809 & \textbf{0.7992} & 0.7816 & 0.7830 & 0.7698 & 0.7681 \\ 
\hline
\end{tabular}
\label{tab:auc_1}
\end{table}

\begin{figure}[H]
\centering
\includegraphics[scale=0.4]{content/images/statExamples-graph_ranks1.png}
\caption{The Nemenyi post-hoc test results.}
\label{fig:ranking_auc_1}
\end{figure}




==> content/chapters/chapter-5/tables/auc-table-2.tex <==
\begin{table*}[htbp]
\small
\caption{Average, standard deviation AUC, and Wilcoxon Signed Rank Test.}
\begin{center}
\begin{tabular}{ccccccc}
\hline
Datasets & ABag-40 & SABag-40 & SBag-40 & Bag-40 & Boost-40 & RandSub-40 \\ 
\hline
\hline
1 & \textbf{0.7923 (0.0500)} & 0.7829 (0.0193) & 0.7816 (0.0770) &  0.7521 (0.0529) &  0.7326 (0.0612) &  0.7573 (0.0215) \\ 
2 & \textbf{0.7390 (0.0194)} & 0.7377 (0.0189) & 0.6988 (0.0307) &  0.7215 (0.0227) &  0.6913 (0.0333) &  0.7217 (0.0243) \\ 
3 & \textbf{1.0000 (0.0000)} & \textbf{1.0000 (0.0000)} & \textbf{1.0000 (0.0000)} & \textbf{ 1.0000 (0.0000)} & \textbf{ 1.0000 (0.0000)} & \textbf{ 1.0000 (0.0000)} \\ 
4 & 0.7309 (0.0343) & 0.7204 (0.0237) & \textbf{0.7314 (0.0282)} &  0.6810 (0.0187) &  0.6611 (0.0252) &  0.6842 (0.0184) \\ 
5 & 0.9592 (0.0168) & 0.9630 (0.0159) & \textbf{0.9669 (0.0127)} &  0.9594 (0.0225) &  0.9472 (0.0182) &  0.9624 (0.0188) \\ 
6 & 0.7368 (0.0188) & \textbf{0.7566 (0.0162)} & 0.7300 (0.0083) &  0.6600 (0.0226) &  0.6750 (0.0072) &  0.6475 (0.0245) \\ 
7 & 0.8722 (0.0497) & \textbf{0.8795 (0.0444)} & 0.8642 (0.0414) &  0.8480 (0.0454) &  0.8356 (0.0325) &  0.8504 (0.0452) \\ 
8 & 0.8855 (0.0495) & \textbf{0.8861 (0.0439)} & 0.8670 (0.0529) &  0.8714 (0.0464) &  0.8226 (0.0347) &  0.8669 (0.0609) \\ 
9 & 0.8917 (0.0190) & \textbf{0.8965 (0.0643)} & 0.8886 (0.0361) &  0.8865 (0.0624) &  0.8223 (0.0520) &  0.8305 (0.0560) \\ 
10 & \textbf{0.9089 (0.0273)} & 0.9045 (0.0248) & 0.9055 (0.0095) &  0.8434 (0.0337) &  0.8239 (0.0305) &  0.8532 (0.0371) \\ 
11 & 0.8047 (0.0967) & \textbf{0.8223 (0.0590)} & 0.7525 (0.0827) &  0.7724 (0.0677) &  0.7130 (0.0842) &  0.7867 (0.0571) \\ 
12 & 0.9483 (0.0573) & 0.9594 (0.0546) & 0.9455 (0.0547) &  0.9589 (0.0540) &  0.9372 (0.0463) & \textbf{ 0.9600 (0.0536)} \\ 
13 & 0.8750 (0.1877) & \textbf{0.8825 (0.1915)} & 0.8708 (0.0982) &  0.7467 (0.1654) &  0.8517 (0.1670) &  0.8017 (0.1662) \\ 
14 & 0.8405 (0.1143) & \textbf{0.8655 (0.0721)} & 0.8155 (0.1194) &  0.8671 (0.1326) &  0.7624 (0.1425) &  0.8671 (0.1326) \\ 
15 & \textbf{0.9978 (0.0045)} & \textbf{0.9978 (0.0045)} & \textbf{0.9978 (0.0045)} &  0.9766 (0.0414) &  0.9955 (0.0055) &  0.9600 (0.0492) \\ 
\hline
Average & 0.8655 (0.0497) & \textbf{0.8703 (0.0435)} & 0.8544 (0.0438) & 0.8363 (0.0526) & 0.8181 (0.0494) & 0.8366 (0.0510) \\ 
\hline
\multicolumn{1}{l}{ABag \textit{p-value}} & NA & 0.9578963 & 0.002606621 & 0.003203245 & 0.0003274792 & 0.002257026 \\ 
\multicolumn{1}{l}{ABag \textit{result}} & ~ & - & + & + & + & + \\ 
\hline
\multicolumn{1}{l}{SABag \textit{p-value}} & 0.04210371 & NA & 0.003159261 & 0.0004935487 & 0.0003274792 & 0.0008084966 \\ 
\multicolumn{1}{l}{SABag \textit{result}} & + & ~ & + & + & + & + \\ 
\hline
\end{tabular}
\end{center}
\label{tab:auc_40}
\end{table*}


==> content/chapters/chapter-5/tables/auc-table.tex <==
% !TEX encoding = ISO88591

\begin{table*}[ht]
\caption{Average, standard deviation AUC, and Wilcoxon Signed Rank Test.}
\begin{center}
\begin{tabular}{ccccccccccccc}

\hline
Dataset & \multicolumn{ 2}{c}{ABag-40} & \multicolumn{ 2}{c}{SABag-40} & \multicolumn{ 2}{c}{SBag-40} & \multicolumn{ 2}{c}{Bag-40} & \multicolumn{ 2}{c}{Boost-40} & \multicolumn{ 2}{c}{RandSub-40} \\ 
\hline
\hline
1 & \textbf{0.7923} & \textbf{0.0500} & 0.7829 & 0.0193 & 0.7816 & 0.0770 & 0.7521 & 0.0529 & 0.7326 & 0.0612 & 0.7573 & 0.0215 \\ 
2 & \textbf{0.7390} & \textbf{0.0194} & 0.7377 & 0.0189 & 0.6988 & 0.0307 & 0.7215 & 0.0227 & 0.6913 & 0.0333 & 0.7217 & 0.0243 \\ 
3 & \textbf{1.0000} & \textbf{0.0000} & \textbf{1.0000} & \textbf{0.0000} & \textbf{1.0000} & \textbf{0.0000} & \textbf{1.0000} & \textbf{0.0000} & \textbf{1.0000} & \textbf{0.0000} & \textbf{1.0000} & \textbf{0.0000} \\ 
4 & 0.7309 & 0.0343 & 0.7204 & 0.0237 & \textbf{0.7314} & \textbf{0.0282} & 0.6810 & 0.0187 & 0.6611 & 0.0252 & 0.6842 & 0.0184 \\ 
5 & 0.9592 & 0.0168 & 0.9630 & 0.0159 & \textbf{0.9669} & \textbf{0.0127} & 0.9594 & 0.0225 & 0.9472 & 0.0182 & 0.9624 & 0.0188 \\ 
6 & 0.7368 & 0.0188 & \textbf{0.7566} & \textbf{0.0162} & 0.7300 & 0.0083 & 0.6600 & 0.0226 & 0.6750 & 0.0072 & 0.6475 & 0.0245 \\ 
7 & 0.8722 & 0.0497 & \textbf{0.8795} & \textbf{0.0444} & 0.8642 & 0.0414 & 0.8480 & 0.0454 & 0.8356 & 0.0325 & 0.8504 & 0.0452 \\ 
8 & 0.8855 & 0.0495 & \textbf{0.8861} & \textbf{0.0439} & 0.8670 & 0.0529 & 0.8714 & 0.0464 & 0.8226 & 0.0347 & 0.8669 & 0.0609 \\ 
9 & 0.8917 & 0.0190 & \textbf{0.8965} & \textbf{0.0643} & 0.8886 & 0.0361 & 0.8865 & 0.0624 & 0.8223 & 0.0520 & 0.8305 & 0.0560 \\ 
10 & \textbf{0.9089} & \textbf{0.0273} & 0.9045 & 0.0248 & 0.9055 & 0.0095 & 0.8434 & 0.0337 & 0.8239 & 0.0305 & 0.8532 & 0.0371 \\ 
11 & 0.8047 & 0.0967 & \textbf{0.8223} & \textbf{0.0590} & 0.7525 & 0.0827 & 0.7724 & 0.0677 & 0.7130 & 0.0842 & 0.7867 & 0.0571 \\ 
12 & 0.9483 & 0.0573 & 0.9594 & 0.0546 & 0.9455 & 0.0547 & 0.9589 & 0.0540 & 0.9372 & 0.0463 & \textbf{0.9600} & \textbf{0.0536} \\ 
13 & 0.8405 & 0.1143 & \textbf{0.8655} & \textbf{0.0721} & 0.8155 & 0.1194 & 0.8671 & 0.1326 & 0.7624 & 0.1425 & 0.8671 & 0.1326 \\ 
14 & 0.8750 & 0.1877 & \textbf{0.8825} & \textbf{0.1915} & 0.8708 & 0.0982 & 0.7467 & 0.1654 & 0.8517 & 0.1670 & 0.8017 & 0.1662 \\ 
15 & \textbf{0.9978} & \textbf{0.0045} & \textbf{0.9978} & \textbf{0.0045} & \textbf{0.9978} & \textbf{0.0045} & 0.9766 & 0.0414 & 0.9955 & 0.0055 & 0.9600 & 0.0492 \\ 
\hline

\multicolumn{1}{c}{Average} & 0.8655 & 0.0497 & \textbf{0.8703} & \textbf{0.0435} & 0.8544 & 0.0438 & 0.8363 & 0.0526 & 0.8181 & 0.0494 & 0.8366 & 0.0510 \\ 
\hline

\multicolumn{1}{l}{ABag \textit{p-value}} & \multicolumn{ 2}{c}{NA} & \multicolumn{ 2}{c}{0.9578963} & \multicolumn{ 2}{c}{0.002606621} & \multicolumn{ 2}{c}{0.003203245} & \multicolumn{ 2}{c}{0.0003274792} & \multicolumn{ 2}{c}{0.002257026} \\ 

\multicolumn{1}{l}{ABag \textit{result}} & \multicolumn{ 2}{c}{NA} & \multicolumn{ 2}{c}{$-$} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{$+$} \\ 
\hline

\multicolumn{1}{l}{SABag \textit{p-value}} & \multicolumn{ 2}{c}{0.04210371} & \multicolumn{ 2}{c}{NA} & \multicolumn{ 2}{c}{0.003159261} & \multicolumn{ 2}{c}{0.0004935487} & \multicolumn{ 2}{c}{0.0003274792} & \multicolumn{ 2}{c}{0.0008084966} \\ 

\multicolumn{1}{l}{SABag \textit{result}} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{NA} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{$+$} \\ 
\hline


\end{tabular}
\end{center}
\label{tab:auc_40}
\end{table*}



==> content/chapters/chapter-5/tables/div-table-2.tex <==
\begin{table*}[htbp]
\small
\caption{Average, standard deviation Entropy Measure $e$, and Wilcoxon Signed Rank Test.}
\begin{center}
\begin{tabular}{cllllll}
\hline
Datasets & \multicolumn{1}{c}{ABag-40} & \multicolumn{1}{c}{SABag-40} & \multicolumn{1}{c}{Sbag-40} & \multicolumn{1}{c}{Bag-40} & \multicolumn{1}{c}{Boost-40} & \multicolumn{1}{c}{RandSub-40} \\ 
\hline
\hline
1 & 0.4445 (0.0560) & 0.4314 (0.0570) & 0.4177 (0.0464) & 0.3786 (0.0531) & 0.1731 (0.1185) & 0.4855 (0.0337) \\ 
2 & 0.4284 (0.0133) & 0.4130 (0.0197) & 0.4303 (0.0174) & 0.4131 (0.0196) & 0.5332 (0.0273) & 0.5336 (0.0257) \\ 
3 & 0.0000 (0.0000) & 0.0000 (0.0000) & 0.0000 (0.0000) & 0.0000 (0.0000) & 0.0000 (0.0000) & 0.0100 (0.0080) \\ 
4 & 0.4342 (0.0230) & 0.3926 (0.0256) & 0.3779 (0.0200) & 0.3410 (0.0029) & 0.6084 (0.0116) & 0.3912 (0.0187) \\ 
5 & 0.1006 (0.0148) & 0.0809 (0.0039) & 0.0849 (0.0059) & 0.0886 (0.0126) & 0.0496 (0.0271) & 0.1506 (0.0045) \\ 
6 & 0.3900 (0.0219) & 0.3774 (0.0248) & 0.3757 (0.0239) & 0.3661 (0.0177) & 0.4756 (0.0261) & 0.3837 (0.0299) \\ 
7 & 0.1542 (0.0361) & 0.1555 (0.0479) & 0.1474 (0.0340) & 0.1456 (0.0337) & 0.0400 (0.0496) & 0.3274 (0.0353) \\ 
8 & 0.1556 (0.0440) & 0.1377 (0.0347) & 0.1174 (0.0203) & 0.1216 (0.0286) & 0.0179 (0.0358) & 0.2435 (0.0297) \\ 
9 & 0.1108 (0.0550) & 0.0894 (0.0235) & 0.0708 (0.0305) & 0.0613 (0.0148) & 0.0000 (0.0000) & 0.1110 (0.0122) \\ 
10 & 0.0767 (0.0076) & 0.0717 (0.0110) & 0.0619 (0.0086) & 0.0825 (0.0086) & 0.1197 (0.0163) & 0.1653 (0.0131) \\ 
11 & 0.1187 (0.0364) & 0.1200 (0.0339) & 0.1089 (0.0361) & 0.1246 (0.0290) & 0.0000 (0.0000) & 0.1881 (0.0226) \\ 
12 & 0.0346 (0.0176) & 0.0309 (0.0148) & 0.0237 (0.0084) & 0.0299 (0.0069) & 0.0000 (0.0000) & 0.0793 (0.0117) \\ 
13 & 0.0684 (0.0299) & 0.0623 (0.0288) & 0.0557 (0.0289) & 0.0944 (0.0312) & 0.0000 (0.0000) & 0.1034 (0.0239) \\ 
14 & 0.0460 (0.0228) & 0.0476 (0.0049) & 0.0253 (0.0125) & 0.0333 (0.0151) & 0.0000 (0.0000) & 0.1048 (0.0288) \\ 
15 & 0.0052 (0.0065) & 0.0020 (0.0035) & 0.0012 (0.0013) & 0.0269 (0.0090) & 0.0000 (0.0000) & 0.0484 (0.0088) \\ 
\hline
Average & 0.1712 (0.0257) & 0.1608 (0.0223) & 0.1533 (0.0196) & 0.1538 (0.0189) & 0.1345 (0.0208) & 0.2217 (0.0204) \\ 
\hline
\multicolumn{1}{l}{ABag p-value} & \multicolumn{1}{c}{NA} & \multicolumn{1}{c}{0.001078881} & \multicolumn{1}{c}{0.0004026381} & \multicolumn{1}{c}{0.02341323} & \multicolumn{1}{c}{0.07781773} & \multicolumn{1}{c}{0.9990406} \\ 
\multicolumn{1}{l}{ABag result} & \multicolumn{1}{c}{NA} & \multicolumn{1}{c}{\$+\$} & \multicolumn{1}{c}{\$+\$} & \multicolumn{1}{c}{\$+\$} & \multicolumn{1}{c}{\$+\$} & \multicolumn{1}{c}{\$-\$} \\ 
\hline
\multicolumn{1}{l}{SABag p-value} & \multicolumn{1}{c}{0.9989211} & \multicolumn{1}{c}{NA} & \multicolumn{1}{c}{0.00529677} & \multicolumn{1}{c}{0.1279943} & \multicolumn{1}{c}{0.1533121} & \multicolumn{1}{c}{0.9997344} \\ 
\multicolumn{1}{l}{SABag-result} & \multicolumn{1}{c}{\$-\$} & \multicolumn{1}{c}{NA} & \multicolumn{1}{c}{\$+\$} & \multicolumn{1}{c}{\$=\$} & \multicolumn{1}{c}{\$=\$} & \multicolumn{1}{c}{\$-\$} \\ 
\hline
\end{tabular}
\end{center}
\label{tab:div_40}
\end{table*}



==> content/chapters/chapter-5/tables/div-table.tex <==
% !TEX encoding = ISO88591

\begin{table*}[ht]
\caption{Average, standard deviation Entropy Measure $e$, and Wilcoxon Signed Rank Test.}
\begin{center}
\begin{tabular}{ccccccccccccc}
\hline
Dataset & \multicolumn{ 2}{c}{ABag-40} & \multicolumn{ 2}{c}{SABag-40} & \multicolumn{ 2}{c}{SBag-40} & \multicolumn{ 2}{c}{Bag-40} & \multicolumn{ 2}{c}{Boost-40} & \multicolumn{ 2}{c}{RandSub-40} \\ 
\hline
\hline
1 & 0.4445 & 0.0560 & 0.4314 & 0.0570 & 0.4177 & 0.0464 & 0.3786 & 0.0531 & 0.1731 & 0.1185 & 0.4855 & 0.0337 \\ 
2 & 0.4284 & 0.0133 & 0.4130 & 0.0197 & 0.4303 & 0.0174 & 0.4131 & 0.0196 & 0.5332 & 0.0273 & 0.5336 & 0.0257 \\ 
3 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0100 & 0.0080 \\ 
4 & 0.4342 & 0.0230 & 0.3926 & 0.0256 & 0.3779 & 0.0200 & 0.3410 & 0.0029 & 0.6084 & 0.0116 & 0.3912 & 0.0187 \\ 
5 & 0.1006 & 0.0148 & 0.0809 & 0.0039 & 0.0849 & 0.0059 & 0.0886 & 0.0126 & 0.0496 & 0.0271 & 0.1506 & 0.0045 \\ 
6 & 0.3900 & 0.0219 & 0.3774 & 0.0248 & 0.3757 & 0.0239 & 0.3661 & 0.0177 & 0.4756 & 0.0261 & 0.3837 & 0.0299 \\ 
7 & 0.1542 & 0.0361 & 0.1555 & 0.0479 & 0.1474 & 0.0340 & 0.1456 & 0.0337 & 0.0400 & 0.0496 & 0.3274 & 0.0353 \\ 
8 & 0.1556 & 0.0440 & 0.1377 & 0.0347 & 0.1174 & 0.0203 & 0.1216 & 0.0286 & 0.0179 & 0.0358 & 0.2435 & 0.0297 \\ 
9 & 0.1108 & 0.0550 & 0.0894 & 0.0235 & 0.0708 & 0.0305 & 0.0613 & 0.0148 & 0.0000 & 0.0000 & 0.1110 & 0.0122 \\ 
10 & 0.0767 & 0.0076 & 0.0717 & 0.0110 & 0.0619 & 0.0086 & 0.0825 & 0.0086 & 0.1197 & 0.0163 & 0.1653 & 0.0131 \\ 
11 & 0.1187 & 0.0364 & 0.1200 & 0.0339 & 0.1089 & 0.0361 & 0.1246 & 0.0290 & 0.0000 & 0.0000 & 0.1881 & 0.0226 \\ 
12 & 0.0346 & 0.0176 & 0.0309 & 0.0148 & 0.0237 & 0.0084 & 0.0299 & 0.0069 & 0.0000 & 0.0000 & 0.0793 & 0.0117 \\ 
13 & 0.0460 & 0.0228 & 0.0476 & 0.0049 & 0.0253 & 0.0125 & 0.0333 & 0.0151 & 0.0000 & 0.0000 & 0.1048 & 0.0288 \\ 
14 & 0.0684 & 0.0299 & 0.0623 & 0.0288 & 0.0557 & 0.0289 & 0.0944 & 0.0312 & 0.0000 & 0.0000 & 0.1034 & 0.0239 \\ 
15 & 0.0052 & 0.0065 & 0.0020 & 0.0035 & 0.0012 & 0.0013 & 0.0269 & 0.0090 & 0.0000 & 0.0000 & 0.0484 & 0.0088 \\ 
\hline
Average & 0.1712 & 0.0257 & 0.1608 & 0.0223 & 0.1533 & 0.0196 & 0.1538 & 0.0189 & 0.1345 & 0.0208 & 0.2217 & 0.0204 \\ 
\hline
\multicolumn{1}{l}{ABag \textit{p-value}} & \multicolumn{ 2}{c}{NA} & \multicolumn{ 2}{c}{0.001078881} & \multicolumn{ 2}{c}{0.0004026381} & \multicolumn{ 2}{c}{0.02341323} & \multicolumn{ 2}{c}{0.07781773} & \multicolumn{ 2}{c}{0.9990406} \\ 
\multicolumn{1}{l}{ABag \textit{result}} & \multicolumn{ 2}{c}{NA} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{$-$} \\ 
\hline
\multicolumn{1}{l}{SABag \textit{p-value}} & \multicolumn{ 2}{c}{0.9989211} & \multicolumn{ 2}{c}{NA} & \multicolumn{ 2}{c}{0.00529677} & \multicolumn{ 2}{c}{0.1279943} & \multicolumn{ 2}{c}{0.1533121} & \multicolumn{ 2}{c}{0.9997344} \\ 
\multicolumn{1}{l}{SABag \textit{result}} & \multicolumn{ 2}{c}{$-$} & \multicolumn{ 2}{c}{NA} & \multicolumn{ 2}{c}{$+$} & \multicolumn{ 2}{c}{$=$} & \multicolumn{ 2}{c}{$=$} & \multicolumn{ 2}{c}{$-$} \\ 
\hline
\end{tabular}
\end{center}
\label{tab:div_40}
\end{table*}



==> content/tables/TABLE_DATASETS.tex <==

\begin{table*}[!htbp]
%\footnotesize
\caption{Summary of the 40 datasets used in the experiments: label, name, number of features, number of samples, and imbalance ratio.}
\resizebox{1.0\textwidth}{!}{
    \begin{tabular}{clrrrcclrrr}
        \hline
        Label & Name                     & \#Feats. & \#Samples & IR   &  & Label & Name                   & \#Feats. & \#Samples & IR    \\
        \hline
        \hline
        1     & glass1                   & 9            & 214        & 1.82 &  & 21    & yeast-2vs4         & 8            & 514        & 9.08  \\
        2     & ecoli0vs1           & 7            & 220        & 1.86 &  & 22    & yeast-05679vs4 & 8            & 528        & 9.35  \\
        3     & wisconsin                & 9            & 683        & 1.86 &  & 23    & vowel0                 & 13           & 988        & 9.98  \\
        4     & pima                     & 8            & 768        & 1.87 &  & 24    & glass-016vs2     & 9            & 192        & 10.29 \\
        5     & iris0                    & 4            & 150        & 2    &  & 25    & glass2                 & 9            & 214        & 11.59 \\
        6     & glass0                   & 9            & 214        & 2.06 &  & 26    & shuttle-c0vsc4       & 9            & 1829       & 13.87 \\
        7     & yeast1                   & 8            & 1484       & 2.46 &  & 27    & yeast-1vs7         & 7            & 459        & 14.3  \\
        8     & vehicle2                 & 18           & 846        & 2.88 &  & 28    & glass4                 & 9            & 214        & 15.47 \\
        9     & vehicle1                 & 18           & 846        & 2.9  &  & 29    & ecoli4                 & 7            & 336        & 15.8  \\
        10    & vehicle3                 & 18           & 846        & 2.99 &  & 30    & page-blocks-13vs4 & 10           & 472        & 15.86 \\
        11    & glass0123vs456 & 9            & 214        & 3.2  &  & 31    & glass-0-1-6\_vs\_5     & 9            & 184        & 19.44 \\
        12    & vehicle0                 & 18           & 846        & 3.25 &  & 32    & shuttle-c2-vs-c4       & 9            & 129        & 20.5  \\
        13    & ecoli1                   & 7            & 336        & 3.36 &  & 33    & yeast-1458vs7   & 8            & 693        & 22.1  \\
        14    & new-thyroid1             & 5            & 215        & 5.14 &  & 34    & glass5                 & 9            & 214        & 22.78 \\
        15    & new-thyroid2             & 5            & 215        & 5.14 &  & 35    & yeast-2vs8         & 8            & 482        & 23.1  \\
        16    & ecoli2                   & 7            & 336        & 5.46 &  & 36    & yeast4                 & 8            & 1484       & 28.1  \\
        17    & segment0                 & 19           & 2308       & 6    &  & 37    & yeast-1289vs7   & 8            & 947        & 30.57 \\
        18    & glass6                   & 9            & 214        & 6.38 &  & 38    & yeast5                 & 8            & 1484       & 32.73 \\
        19    & yeast3                   & 8            & 1484       & 8.1  &  & 39    & ecoli-0137vs26 & 7            & 281        & 39.14 \\
        20    & ecoli3                   & 7            & 336        & 8.6  &  & 40    & yeast6                 & 8            & 1484       & 41.4 \\
        \hline
\end{tabular}
}
\label{tab:datasets}
\end{table*}


==> content/tables/TABLE_DATASETS_S.tex <==

\begin{table}[htbp]
%\footnotesize
\begin{center}
\caption{Summary of the 40 datasets used in the experiments: label, name, number of features, number of samples, and imbalance ratio. (From \cite{dfp:2017})}
\label{tab:datasets}
%\resizebox{1.0\textwidth}{!}{
    \begin{tabular}{clrrr}
        \hline
        
Label & Name            & \#Feats. & \#Samples & IR \\
        \hline
        \hline
1     & glass1          & 9     & 214        & 1.82 \\
2     & ecoli0vs1       & 7     & 220        & 1.86 \\
3     & wisconsin       & 9     & 683        & 1.86 \\
4     & pima            & 8     & 768        & 1.87 \\ 
5     & iris0           & 4     & 150        & 2.00 \\
6     & glass0          & 9     & 214        & 2.06 \\
7     & yeast1          & 8     & 1484       & 2.46 \\ 
8     & vehicle2        & 18    & 846        & 2.88 \\ 
9     & vehicle1        & 18    & 846        & 2.9  \\
10    & vehicle3        & 18    & 846        & 2.99 \\ 
11    & glass0123vs456  & 9     & 214        & 3.2  \\ 
12    & vehicle0        & 18    & 846        & 3.25 \\ 
13    & ecoli1          & 7     & 336        & 3.36 \\ 
14    & new-thyroid1    & 5     & 215        & 5.14 \\ 
15    & new-thyroid2    & 5     & 215        & 5.14 \\
16    & ecoli2          & 7     & 336        & 5.46 \\
17    & segment0        & 19    & 2308       & 6.00 \\
18    & glass6          & 9     & 214        & 6.38 \\
19    & yeast3          & 8     & 1484       & 8.10 \\
20    & ecoli3          & 7     & 336        & 8.60 \\ 
21    & yeast-2vs4      & 8     & 514        & 9.08 \\
22    & yeast-05679vs4  & 8     & 528        & 9.35 \\
23    & vowel0          & 13    & 988        & 9.98 \\
24    & glass-016vs2    & 9     & 192        & 10.29 \\
25    & glass2          & 9     & 214        & 11.59 \\
26    & shuttle-c0vsc4  & 9     & 1829       & 13.87 \\
27    & yeast-1vs7      & 7     & 459        & 14.30 \\
28    & glass4          & 9     & 214        & 15.47 \\
29    & ecoli4          & 7     & 336        & 15.80 \\
30    & page-blocks-13vs4   & 10& 472        & 15.86 \\
31    & glass-0-1-6\_vs\_5  & 9 & 184        & 19.44 \\
32    & shuttle-c2-vs-c4    & 9 & 129        & 20.50 \\
33    & yeast-1458vs7   & 8     & 693        & 22.10 \\
34    & glass5          & 9     & 214        & 22.78 \\
35    & yeast-2vs8      & 8     & 482        & 23.10 \\
36    & yeast4          & 8     & 1484       & 28.10 \\
37    & yeast-1289vs7   & 8     & 947        & 30.57 \\
38    & yeast5          & 8     & 1484       & 32.73 \\
39    & ecoli-0137vs26  & 7     & 281        & 39.14 \\
40    & yeast6          & 8     & 1484       & 41.40 \\
        \hline
\end{tabular}
%}%resizebox
\end{center}
\end{table}


==> content/tables/TABLE_DES.tex <==


\begin{table}
\begin{center}
\caption{
    Dynamic selection techniques considered in the experiment.
}
\label{tab:dsexp}
%\scriptsize
%\resizebox{1.0\textwidth}{!}{
\begin{tabular}{lll}
\hline
Technique & Category & Reference \\
\hline
\hline
DCS & & \\
Overall Local Accuracy (OLA)        & Accuracy      & Woods et al. \cite{dcs_la:1996} \\
Local Class Accuracy (LCA)          & Accuracy      & Woods et al. \cite{dcs_la:1996} \\
A Priori (APri)                     & Probabilistic &  Giacinto et al. \cite{dcs_la:1999} \\
A Posteriori (APos)                 & Probabilistic &  Giacinto et al. \cite{dcs_la:1999} \\
Multiple Classifier Behavior (MCB)  & Behavior      & Giacinto et al. \cite{mcb:2001} \\
DES & & \\
Dynamic Selection KNN (DSKNN)       & Diversity     & Santana et al. \cite{dsknn:2006} \\
K-Nearests Oracles Union (KNORA-U)      & Oracle        & Ko et al. \cite{des:2008} \\
K-Nearests Oracles Eliminate (KNORA-E)  & Oracle        & Ko et al. \cite{des:2008} \\
\hline
\end{tabular}
%}
\end{center}
\end{table}



==> content/tables/TABLE_DES_S.tex <==
\begin{table}
\begin{center}
\caption{
    Dynamic selection techniques considered in the experiment.
}
\label{tab:dsexp}
%\scriptsize
%\resizebox{1.0\textwidth}{!}{
\begin{tabular}{lll}
\hline
Technique                               & Category      & Reference         \\
\hline
\hline
DCS                                     &               &                   \\
Overall Local Accuracy (OLA)            & Accuracy      & \cite{dcs_la:1996}\\
Local Class Accuracy (LCA)              & Accuracy      & \cite{dcs_la:1996}\\
A Priori (APri)                         & Probabilistic & \cite{dcs_la:1999}\\
A Posteriori (APos)                     & Probabilistic & \cite{dcs_la:1999}\\
Multiple Classifier Behavior (MCB)      & Behavior      & \cite{mcb:2001}   \\
DES                                     &               &                   \\
Dynamic Selection KNN (DSKNN)           & Diversity     & \cite{dsknn:2006} \\
K-Nearests Oracles Union (KNORA-U)      & Oracle        & \cite{des:2008}   \\
K-Nearests Oracles Eliminate (KNORA-E)  & Oracle        & \cite{des:2008}   \\
\hline
\end{tabular}
%}
\end{center}
\end{table}



==> content/tables/TABLE_FULL.tex <==
\begin{table*}[ht]
    \begin{center}
    \caption{
        Mean and standard deviation AUC of KNORA-B, KNORA-BI,
        KNORA-E, KNORA-U, DSKNN, OLA, LCA, A Priori, A Posteriori,
        MCB, Bagging, Single Best Classifier and the Oracle.
        Best results for each dataset are in bold.
        %and significantly better results
        %are marked with $\bullet$ (\textit{p-value} $\le .10$) and 
        %$\bullet\bullet$ (\textit{p-value} $\le .05$), 
        %where \textit{p-value} is obtained with the 
        %Wilcoxon Signed Rank Test.
    }
    \label{tab:results}
    \resizebox{1.0\textwidth}{!}{
%\begin{tabular}{llllllllllllll}
\begin{tabular}{cccccccccccccc}
    \hline
Dataset &                   KNORA-B &                  KNORA-BI &                   KNORA-E &                   KNORA-U &                     DSKNN &                       OLA &                       LCA &                      APRI &                      APOS &                       MCB &                       BAG &               SB &           Oracle \\
    \hline
    \hline
      1 &           .6259(.0571) &           .6430(.0767) &           .6437(.0458) &           .5931(.0502) &           .6377(.0477) &           .6049(.0879) &           .6248(.0515) &  \textbf{.6782(.0352)} &           .6318(.0625) &           .5226(.0368) &           .5274(.0419) &  .7095(.0652) &  1.000(.0000) \\
      2 &           .9702(.0219) &           .9702(.0219) &           .9702(.0219) &  \textbf{.9764(.0249)} &           .9702(.0219) &           .9499(.0299) &           .9311(.0230) &           .9570(.0294) &           .9507(.0370) &  \textbf{.9764(.0249)} &  \textbf{.9764(.0249)} &  .9867(.0163) &  1.000(.0000) \\
      3 &           .9425(.0195) &           .9487(.0193) &           .9478(.0147) &           .9675(.0086) &           .9603(.0120) &           .9475(.0219) &           .9545(.0173) &           .9518(.0254) &           .9586(.0163) &  \textbf{.9717(.0100)} &  \textbf{.9717(.0079)} &  .9847(.0036) &  .9957(.0040) \\
      4 &           .6692(.0188) &           .6752(.0139) &           .6741(.0364) &           .7205(.0326) &           .6665(.0390) &           .6640(.0144) &           .6437(.0281) &           .6661(.0226) &           .6775(.0246) &           .7194(.0268) &  \textbf{.7232(.0215)} &  .7773(.0186) &  .9981(.0038) \\
      5 &  \textbf{1.000(.0000)} &  \textbf{1.000(.0000)} &  \textbf{1.000(.0000)} &  \textbf{1.000(.0000)} &  \textbf{1.000(.0000)} &           .9900(.0200) &  \textbf{1.000(.0000)} &  \textbf{1.000(.0000)} &  \textbf{1.000(.0000)} &  \textbf{1.000(.0000)} &  \textbf{1.000(.0000)} &  1.000(.0000) &  1.000(.0000) \\
      6 &           .7026(.0283) &           .6722(.0477) &           .6994(.0374) &           .6952(.0748) &           .6926(.0261) &           .7140(.0735) &           .6860(.0325) &           .7138(.0787) &  \textbf{.7355(.0496)} &           .6299(.1079) &           .6768(.0611) &  .8046(.0413) &  1.000(.0000) \\
      7 &           .6401(.0261) &           .6653(.0289) &           .6501(.0245) &           .6575(.0178) &  \textbf{.6768(.0119)} &           .6625(.0257) &           .6615(.0173) &           .6694(.0210) &           .6658(.0235) &           .6231(.0356) &           .6225(.0234) &  .7298(.0287) &  .9979(.0026) \\
      8 &           .9463(.0195) &           .9516(.0074) &  \textbf{.9548(.0105)} &           .9281(.0214) &           .9494(.0111) &           .9464(.0092) &           .8539(.0305) &           .9425(.0104) &           .9320(.0168) &           .9043(.0345) &           .9204(.0220) &  .9375(.0158) &  1.000(.0000) \\
      9 &           .6896(.0296) &  \textbf{.7309(.0254)} &           .6922(.0282) &           .6555(.0348) &           .6813(.0514) &           .7007(.0342) &           .6258(.0430) &           .6432(.0361) &           .6480(.0282) &           .6340(.0554) &           .6610(.0536) &  .7573(.0111) &  1.000(.0000) \\
     10 &           .7043(.0376) &  \textbf{.7182(.0398)} &           .7089(.0358) &           .6269(.0337) &           .6986(.0305) &           .6910(.0327) &           .6501(.0319) &           .6602(.0297) &           .6831(.0343) &           .6007(.0472) &           .5971(.0376) &  .7285(.0243) &  .9929(.0143) \\
     11 &           .8834(.0641) &           .8904(.0521) &           .8866(.0644) &           .9003(.0702) &           .8921(.0682) &  \textbf{.9194(.0618)} &           .8452(.0773) &           .8521(.0571) &           .8743(.0605) &           .9003(.0702) &           .9021(.0748) &  .9655(.0230) &  .9969(.0063) \\
     12 &           .9435(.0107) &           .9469(.0133) &           .9427(.0093) &  \textbf{.9525(.0139)} &           .9426(.0098) &           .9474(.0254) &           .8316(.0581) &           .9297(.0130) &           .9064(.0436) &           .9473(.0106) &           .9416(.0160) &  .9768(.0114) &  1.000(.0000) \\
     13 &           .8107(.0206) &           .8199(.0208) &           .8145(.0180) &           .8312(.0353) &  \textbf{.8683(.0321)} &           .8410(.0332) &           .8359(.0485) &           .8446(.0256) &           .8379(.0398) &           .8249(.0553) &           .8273(.0541) &  .9198(.0302) &  1.000(.0000) \\
     14 &           .9687(.0331) &           .9687(.0331) &           .9687(.0331) &           .9258(.0455) &           .9659(.0309) &           .9516(.0540) &           .7857(.0782) &           .8829(.0553) &           .8429(.0535) &           .9258(.0455) &  \textbf{.9829(.0277)} &  1.000(.0000) &  1.000(.0000) \\
     15 &  \textbf{.9687(.0331)} &  \textbf{.9687(.0331)} &  \textbf{.9687(.0331)} &  \textbf{.9687(.0331)} &  \textbf{.9687(.0331)} &           .9429(.0286) &           .7714(.0948) &           .8401(.0667) &           .8143(.0969) &           .9544(.0553) &           .9544(.0553) &  1.000(.0000) &  1.000(.0000) \\
     16 &           .8447(.0617) &           .8536(.1129) &           .8547(.0601) &           .8661(.0710) &           .8926(.0717) &           .8785(.0689) &           .8903(.0541) &           .8978(.0630) &  \textbf{.9008(.0499)} &           .7862(.0646) &           .8162(.0420) &  .9279(.0316) &  .9818(.0223) \\
     17 &           .9914(.0088) &           .9912(.0086) &           .9917(.0090) &           .9907(.0071) &           .9891(.0074) &  \textbf{.9922(.0081)} &           .9823(.0150) &           .9886(.0101) &  \textbf{.9922(.0071)} &           .9907(.0071) &           .9907(.0071) &  .9929(.0067) &  1.000(.0000) \\
     18 &           .8659(.0774) &           .8605(.0834) &           .8686(.0747) &  \textbf{.9032(.0750)} &           .8659(.0774) &           .8523(.0916) &           .8617(.0640) &           .8698(.0638) &           .8298(.0337) &  \textbf{.9032(.0750)} &           .8352(.0356) &  .9644(.0335) &  1.000(.0000) \\
     19 &           .8214(.0179) &  \textbf{.8564(.0338)} &           .8173(.0207) &           .8425(.0614) &           .8516(.0265) &           .8493(.0417) &           .8062(.0336) &           .8269(.0540) &           .8171(.0387) &           .8263(.0604) &           .8064(.0746) &  .9251(.0194) &  1.000(.0000) \\
     20 &           .7542(.1127) &  \textbf{.8223(.0943)} &           .7718(.1044) &           .7690(.0961) &           .7817(.1044) &           .7893(.0984) &           .7421(.0479) &           .7784(.0526) &           .7834(.0206) &           .7296(.1260) &           .7372(.1096) &  .9374(.0434) &  1.000(.0000) \\
     21 &           .8389(.0763) &           .8302(.0756) &  \textbf{.8410(.0772)} &           .7922(.0648) &           .8181(.0737) &           .7895(.1308) &           .7551(.0942) &           .7831(.0756) &           .7840(.0985) &           .7722(.0510) &           .8295(.0674) &  .9118(.0325) &  .9609(.0196) \\
     22 &           .7019(.0836) &           .7325(.0520) &           .6908(.0914) &           .6610(.0509) &  \textbf{.7340(.1099)} &           .7146(.0924) &           .6116(.1074) &           .6601(.0984) &           .6479(.0752) &           .6620(.0274) &           .6740(.0513) &  .8651(.0587) &  .9600(.0374) \\
     23 &           .9239(.0527) &           .9239(.0527) &           .9244(.0526) &           .8244(.0423) &           .8972(.0562) &  \textbf{.9422(.0316)} &           .6194(.0594) &           .9367(.0365) &           .9050(.0227) &           .8228(.0292) &           .8617(.0452) &  .9549(.0214) &  1.000(.0000) \\
     24 &           .5071(.0965) &  \textbf{.5640(.1263)} &           .4993(.0593) &           .5000(.0000) &           .5000(.0000) &           .4914(.0114) &           .5000(.0000) &           .4943(.0070) &           .4971(.0057) &           .5000(.0000) &           .5000(.0000) &  .6814(.0799) &  1.000(.0000) \\
     25 &           .5459(.0834) &  \textbf{.5967(.1996)} &           .5259(.0949) &           .5000(.0000) &           .5000(.0000) &           .4745(.0140) &           .5000(.0000) &           .4974(.0051) &           .4974(.0051) &           .5000(.0000) &           .5000(.0000) &  .7556(.1140) &  1.000(.0000) \\
     26 &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  .9960(.0080) &  .9960(.0080) \\
     27 &           .6042(.0759) &           .5964(.0655) &  \textbf{.6135(.0772)} &           .5667(.0624) &           .5298(.0390) &           .6038(.0602) &           .5167(.0333) &           .5333(.0408) &           .5167(.0333) &           .5655(.0636) &           .5655(.0636) &  .8266(.0375) &  1.000(.0000) \\
     28 &           .7684(.1632) &           .7684(.1632) &           .7684(.1632) &           .5617(.0862) &           .6684(.1803) &  \textbf{.7992(.1922)} &           .5000(.0000) &           .6450(.1344) &           .6283(.1850) &           .5592(.0881) &           .5567(.0899) &  .9777(.0162) &  1.000(.0000) \\
     29 &           .9187(.0573) &           .9187(.0573) &           .9187(.0573) &  \textbf{.9203(.0555)} &           .9187(.0537) &           .8655(.1314) &           .7000(.1275) &           .8750(.0791) &           .8750(.0791) &  \textbf{.9203(.0555)} &  \textbf{.9203(.0555)} &  .9968(.0063) &  1.000(.0000) \\
     30 &           .9377(.0497) &           .9354(.0470) &  \textbf{.9399(.0499)} &           .7288(.1163) &           .7300(.1157) &           .8866(.0282) &           .6289(.0998) &           .8000(.0881) &           .8355(.0764) &           .7277(.1262) &           .7144(.1283) &  .9504(.0173) &  1.000(.0000) \\
     31 &  \textbf{.9800(.0249)} &  \textbf{.9800(.0249)} &  \textbf{.9800(.0249)} &           .5000(.0000) &           .4971(.0057) &           .9771(.0232) &           .5000(.0000) &           .5471(.1016) &           .6000(.2000) &           .5000(.0000) &           .5500(.1000) &  .9771(.0146) &  1.000(.0000) \\
     32 &           .9460(.0983) &           .9460(.0983) &           .9460(.0983) &           .9460(.0983) &           .9460(.0983) &  \textbf{.9960(.0080)} &           .5000(.0000) &           .7500(.2236) &           .6500(.2000) &           .8960(.1982) &           .9460(.0983) &  1.000(.0000) &  1.000(.0000) \\
     33 &           .6197(.0650) &  \textbf{.6298(.0643)} &           .5879(.0360) &           .5000(.0000) &           .5000(.0000) &           .4977(.0019) &           .4992(.0015) &           .4992(.0015) &           .4992(.0015) &           .5000(.0000) &           .5000(.0000) &  .6828(.0370) &  1.000(.0000) \\
     34 &           .8329(.1937) &  \textbf{.8707(.1923)} &           .7927(.2393) &           .5000(.0000) &           .5500(.1000) &           .7878(.2355) &           .5000(.0000) &           .6000(.2000) &           .6000(.2000) &           .5000(.0000) &           .5500(.1000) &  .9683(.0226) &  1.000(.0000) \\
     35 &           .7435(.0724) &           .7217(.0566) &           .7457(.0740) &           .7489(.0773) &           .7489(.0773) &           .7446(.0740) &           .5250(.0500) &           .7500(.0791) &           .7250(.0500) &           .7489(.0773) &  \textbf{.7739(.0924)} &  .8239(.0626) &  .8750(.1118) \\
     36 &           .6975(.0724) &  \textbf{.7449(.0762)} &           .6902(.0828) &           .5771(.0238) &           .5870(.0661) &           .6442(.0705) &           .5200(.0400) &           .5690(.0674) &           .5400(.0374) &           .5652(.0465) &           .5587(.0198) &  .8427(.0281) &  .9400(.0583) \\
     37 &           .5514(.0630) &           .5263(.0600) &  \textbf{.5541(.0643)} &           .5167(.0333) &           .5333(.0408) &           .5301(.0425) &           .5000(.0000) &           .5167(.0333) &           .5000(.0000) &           .5333(.0408) &           .5328(.0413) &  .7917(.0331) &  .9833(.0333) \\
     38 &           .7406(.1110) &           .8167(.0915) &           .7542(.1141) &           .7097(.0932) &  \textbf{.8569(.0588)} &           .7934(.0823) &           .7247(.0121) &           .8045(.0563) &           .7580(.0243) &           .6535(.0919) &           .7118(.0786) &  .9854(.0042) &  1.000(.0000) \\
     39 &           .8463(.1996) &           .8463(.1996) &           .8463(.1996) &           .8463(.1996) &           .8463(.1996) &           .7427(.2217) &           .5000(.0000) &           .7981(.1876) &           .7500(.2236) &           .8463(.1996) &  \textbf{.8481(.2010)} &  .9209(.1024) &  .9500(.1000) \\
     40 &  \textbf{.8022(.0858)} &           .7970(.0843) &           .7893(.0837) &           .6411(.0792) &           .6945(.0516) &           .7618(.0949) &           .6119(.0719) &           .6690(.0728) &           .6258(.0820) &           .5840(.0295) &           .5700(.0631) &  .9064(.0721) &  .9714(.0571) \\
\hline
   Mean &           .8062(.0608) &  \textbf{.8174(.0640)} &           .8058(.0608) &           .7577(.0475) &           .7751(.0512) &           .7968(.0604) &           .6923(.0388) &           .7579(.0586) &           .7478(.0586) &           .7431(.0520) &           .7532(.0524) &  .8960(.0298) &  .9900(.0120) \\
\hline
Wilcox &                         1 &                   .99736 &                  .782792 &                 .0024846 &                 .0937058 &                  .136656 &               $9.15 \times e^{-7}$ &                .00105434 &               $9.68 \times e{-5}$ &               $3.86 \times e^{-5}$ &                 .0001961 &                1 &                1 \\
 Wilcox &                         NA &                         - &                         = &                         + &                         = &                         = &                         + &                         + &                         + &                         + &                         + &                - &                - \\
Wilcox &                .00282207 &                         1 &                 .0184106 &                .00031885 &                .00683614 &                .00376574 &               $2.82 \times e^{-7}$ &               $3.76 \times e^{-5}$ &               $4.86 \times e^{-6}$ &                $1.78 \times e^{-5}$ &               .000138562 &                1 &                1 \\
 Wilcox &                         + &                         NA &                         + &                         + &                         + &                         + &                         + &                         + &                         + &                         + &                         + &                - &                - \\
\hline
\end{tabular}
}
\end{center}
\end{table*}


==> content/tables/TABLE_FULL_H.tex <==
\newgeometry{margin=1cm} % modify this if you need even more space
\begin{landscape}
\begin{table}
    \begin{center}
    \caption{
        Mean and standard deviation AUC of KNORA-B, KNORA-BI,
        KNORA-E, KNORA-U, DSKNN, OLA, LCA, A Priori, A Posteriori,
        MCB, Bagging, Single Best Classifier and the Oracle.
        Best results for each dataset are in bold.
        %and significantly better results
        %are marked with $\bullet$ (\textit{p-value} $\le .10$) and 
        %$\bullet\bullet$ (\textit{p-value} $\le .05$), 
        %where \textit{p-value} is obtained with the 
        %Wilcoxon Signed Rank Test.
    }
    \label{tab:results}
    \resizebox{1.0\textwidth}{!}{
%\begin{tabular}{llllllllllllll}
\begin{tabular}{cccccccccccccc}
    \hline
Dataset &                   KNORA-B &                  KNORA-BI &                   KNORA-E &                   KNORA-U &                     DSKNN &                       OLA &                       LCA &                      APRI &                      APOS &                       MCB &                       BAG &               SB &           Oracle \\
    \hline
    \hline
      1 &           .6259(.0571) &           .6430(.0767) &           .6437(.0458) &           .5931(.0502) &           .6377(.0477) &           .6049(.0879) &           .6248(.0515) &  \textbf{.6782(.0352)} &           .6318(.0625) &           .5226(.0368) &           .5274(.0419) &  .7095(.0652) &  1.000(.0000) \\
      2 &           .9702(.0219) &           .9702(.0219) &           .9702(.0219) &  \textbf{.9764(.0249)} &           .9702(.0219) &           .9499(.0299) &           .9311(.0230) &           .9570(.0294) &           .9507(.0370) &  \textbf{.9764(.0249)} &  \textbf{.9764(.0249)} &  .9867(.0163) &  1.000(.0000) \\
      3 &           .9425(.0195) &           .9487(.0193) &           .9478(.0147) &           .9675(.0086) &           .9603(.0120) &           .9475(.0219) &           .9545(.0173) &           .9518(.0254) &           .9586(.0163) &  \textbf{.9717(.0100)} &  \textbf{.9717(.0079)} &  .9847(.0036) &  .9957(.0040) \\
      4 &           .6692(.0188) &           .6752(.0139) &           .6741(.0364) &           .7205(.0326) &           .6665(.0390) &           .6640(.0144) &           .6437(.0281) &           .6661(.0226) &           .6775(.0246) &           .7194(.0268) &  \textbf{.7232(.0215)} &  .7773(.0186) &  .9981(.0038) \\
      5 &  \textbf{1.000(.0000)} &  \textbf{1.000(.0000)} &  \textbf{1.000(.0000)} &  \textbf{1.000(.0000)} &  \textbf{1.000(.0000)} &           .9900(.0200) &  \textbf{1.000(.0000)} &  \textbf{1.000(.0000)} &  \textbf{1.000(.0000)} &  \textbf{1.000(.0000)} &  \textbf{1.000(.0000)} &  1.000(.0000) &  1.000(.0000) \\
      6 &           .7026(.0283) &           .6722(.0477) &           .6994(.0374) &           .6952(.0748) &           .6926(.0261) &           .7140(.0735) &           .6860(.0325) &           .7138(.0787) &  \textbf{.7355(.0496)} &           .6299(.1079) &           .6768(.0611) &  .8046(.0413) &  1.000(.0000) \\
      7 &           .6401(.0261) &           .6653(.0289) &           .6501(.0245) &           .6575(.0178) &  \textbf{.6768(.0119)} &           .6625(.0257) &           .6615(.0173) &           .6694(.0210) &           .6658(.0235) &           .6231(.0356) &           .6225(.0234) &  .7298(.0287) &  .9979(.0026) \\
      8 &           .9463(.0195) &           .9516(.0074) &  \textbf{.9548(.0105)} &           .9281(.0214) &           .9494(.0111) &           .9464(.0092) &           .8539(.0305) &           .9425(.0104) &           .9320(.0168) &           .9043(.0345) &           .9204(.0220) &  .9375(.0158) &  1.000(.0000) \\
      9 &           .6896(.0296) &  \textbf{.7309(.0254)} &           .6922(.0282) &           .6555(.0348) &           .6813(.0514) &           .7007(.0342) &           .6258(.0430) &           .6432(.0361) &           .6480(.0282) &           .6340(.0554) &           .6610(.0536) &  .7573(.0111) &  1.000(.0000) \\
     10 &           .7043(.0376) &  \textbf{.7182(.0398)} &           .7089(.0358) &           .6269(.0337) &           .6986(.0305) &           .6910(.0327) &           .6501(.0319) &           .6602(.0297) &           .6831(.0343) &           .6007(.0472) &           .5971(.0376) &  .7285(.0243) &  .9929(.0143) \\
     11 &           .8834(.0641) &           .8904(.0521) &           .8866(.0644) &           .9003(.0702) &           .8921(.0682) &  \textbf{.9194(.0618)} &           .8452(.0773) &           .8521(.0571) &           .8743(.0605) &           .9003(.0702) &           .9021(.0748) &  .9655(.0230) &  .9969(.0063) \\
     12 &           .9435(.0107) &           .9469(.0133) &           .9427(.0093) &  \textbf{.9525(.0139)} &           .9426(.0098) &           .9474(.0254) &           .8316(.0581) &           .9297(.0130) &           .9064(.0436) &           .9473(.0106) &           .9416(.0160) &  .9768(.0114) &  1.000(.0000) \\
     13 &           .8107(.0206) &           .8199(.0208) &           .8145(.0180) &           .8312(.0353) &  \textbf{.8683(.0321)} &           .8410(.0332) &           .8359(.0485) &           .8446(.0256) &           .8379(.0398) &           .8249(.0553) &           .8273(.0541) &  .9198(.0302) &  1.000(.0000) \\
     14 &           .9687(.0331) &           .9687(.0331) &           .9687(.0331) &           .9258(.0455) &           .9659(.0309) &           .9516(.0540) &           .7857(.0782) &           .8829(.0553) &           .8429(.0535) &           .9258(.0455) &  \textbf{.9829(.0277)} &  1.000(.0000) &  1.000(.0000) \\
     15 &  \textbf{.9687(.0331)} &  \textbf{.9687(.0331)} &  \textbf{.9687(.0331)} &  \textbf{.9687(.0331)} &  \textbf{.9687(.0331)} &           .9429(.0286) &           .7714(.0948) &           .8401(.0667) &           .8143(.0969) &           .9544(.0553) &           .9544(.0553) &  1.000(.0000) &  1.000(.0000) \\
     16 &           .8447(.0617) &           .8536(.1129) &           .8547(.0601) &           .8661(.0710) &           .8926(.0717) &           .8785(.0689) &           .8903(.0541) &           .8978(.0630) &  \textbf{.9008(.0499)} &           .7862(.0646) &           .8162(.0420) &  .9279(.0316) &  .9818(.0223) \\
     17 &           .9914(.0088) &           .9912(.0086) &           .9917(.0090) &           .9907(.0071) &           .9891(.0074) &  \textbf{.9922(.0081)} &           .9823(.0150) &           .9886(.0101) &  \textbf{.9922(.0071)} &           .9907(.0071) &           .9907(.0071) &  .9929(.0067) &  1.000(.0000) \\
     18 &           .8659(.0774) &           .8605(.0834) &           .8686(.0747) &  \textbf{.9032(.0750)} &           .8659(.0774) &           .8523(.0916) &           .8617(.0640) &           .8698(.0638) &           .8298(.0337) &  \textbf{.9032(.0750)} &           .8352(.0356) &  .9644(.0335) &  1.000(.0000) \\
     19 &           .8214(.0179) &  \textbf{.8564(.0338)} &           .8173(.0207) &           .8425(.0614) &           .8516(.0265) &           .8493(.0417) &           .8062(.0336) &           .8269(.0540) &           .8171(.0387) &           .8263(.0604) &           .8064(.0746) &  .9251(.0194) &  1.000(.0000) \\
     20 &           .7542(.1127) &  \textbf{.8223(.0943)} &           .7718(.1044) &           .7690(.0961) &           .7817(.1044) &           .7893(.0984) &           .7421(.0479) &           .7784(.0526) &           .7834(.0206) &           .7296(.1260) &           .7372(.1096) &  .9374(.0434) &  1.000(.0000) \\
     21 &           .8389(.0763) &           .8302(.0756) &  \textbf{.8410(.0772)} &           .7922(.0648) &           .8181(.0737) &           .7895(.1308) &           .7551(.0942) &           .7831(.0756) &           .7840(.0985) &           .7722(.0510) &           .8295(.0674) &  .9118(.0325) &  .9609(.0196) \\
     22 &           .7019(.0836) &           .7325(.0520) &           .6908(.0914) &           .6610(.0509) &  \textbf{.7340(.1099)} &           .7146(.0924) &           .6116(.1074) &           .6601(.0984) &           .6479(.0752) &           .6620(.0274) &           .6740(.0513) &  .8651(.0587) &  .9600(.0374) \\
     23 &           .9239(.0527) &           .9239(.0527) &           .9244(.0526) &           .8244(.0423) &           .8972(.0562) &  \textbf{.9422(.0316)} &           .6194(.0594) &           .9367(.0365) &           .9050(.0227) &           .8228(.0292) &           .8617(.0452) &  .9549(.0214) &  1.000(.0000) \\
     24 &           .5071(.0965) &  \textbf{.5640(.1263)} &           .4993(.0593) &           .5000(.0000) &           .5000(.0000) &           .4914(.0114) &           .5000(.0000) &           .4943(.0070) &           .4971(.0057) &           .5000(.0000) &           .5000(.0000) &  .6814(.0799) &  1.000(.0000) \\
     25 &           .5459(.0834) &  \textbf{.5967(.1996)} &           .5259(.0949) &           .5000(.0000) &           .5000(.0000) &           .4745(.0140) &           .5000(.0000) &           .4974(.0051) &           .4974(.0051) &           .5000(.0000) &           .5000(.0000) &  .7556(.1140) &  1.000(.0000) \\
     26 &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  \textbf{.9960(.0080)} &  .9960(.0080) &  .9960(.0080) \\
     27 &           .6042(.0759) &           .5964(.0655) &  \textbf{.6135(.0772)} &           .5667(.0624) &           .5298(.0390) &           .6038(.0602) &           .5167(.0333) &           .5333(.0408) &           .5167(.0333) &           .5655(.0636) &           .5655(.0636) &  .8266(.0375) &  1.000(.0000) \\
     28 &           .7684(.1632) &           .7684(.1632) &           .7684(.1632) &           .5617(.0862) &           .6684(.1803) &  \textbf{.7992(.1922)} &           .5000(.0000) &           .6450(.1344) &           .6283(.1850) &           .5592(.0881) &           .5567(.0899) &  .9777(.0162) &  1.000(.0000) \\
     29 &           .9187(.0573) &           .9187(.0573) &           .9187(.0573) &  \textbf{.9203(.0555)} &           .9187(.0537) &           .8655(.1314) &           .7000(.1275) &           .8750(.0791) &           .8750(.0791) &  \textbf{.9203(.0555)} &  \textbf{.9203(.0555)} &  .9968(.0063) &  1.000(.0000) \\
     30 &           .9377(.0497) &           .9354(.0470) &  \textbf{.9399(.0499)} &           .7288(.1163) &           .7300(.1157) &           .8866(.0282) &           .6289(.0998) &           .8000(.0881) &           .8355(.0764) &           .7277(.1262) &           .7144(.1283) &  .9504(.0173) &  1.000(.0000) \\
     31 &  \textbf{.9800(.0249)} &  \textbf{.9800(.0249)} &  \textbf{.9800(.0249)} &           .5000(.0000) &           .4971(.0057) &           .9771(.0232) &           .5000(.0000) &           .5471(.1016) &           .6000(.2000) &           .5000(.0000) &           .5500(.1000) &  .9771(.0146) &  1.000(.0000) \\
     32 &           .9460(.0983) &           .9460(.0983) &           .9460(.0983) &           .9460(.0983) &           .9460(.0983) &  \textbf{.9960(.0080)} &           .5000(.0000) &           .7500(.2236) &           .6500(.2000) &           .8960(.1982) &           .9460(.0983) &  1.000(.0000) &  1.000(.0000) \\
     33 &           .6197(.0650) &  \textbf{.6298(.0643)} &           .5879(.0360) &           .5000(.0000) &           .5000(.0000) &           .4977(.0019) &           .4992(.0015) &           .4992(.0015) &           .4992(.0015) &           .5000(.0000) &           .5000(.0000) &  .6828(.0370) &  1.000(.0000) \\
     34 &           .8329(.1937) &  \textbf{.8707(.1923)} &           .7927(.2393) &           .5000(.0000) &           .5500(.1000) &           .7878(.2355) &           .5000(.0000) &           .6000(.2000) &           .6000(.2000) &           .5000(.0000) &           .5500(.1000) &  .9683(.0226) &  1.000(.0000) \\
     35 &           .7435(.0724) &           .7217(.0566) &           .7457(.0740) &           .7489(.0773) &           .7489(.0773) &           .7446(.0740) &           .5250(.0500) &           .7500(.0791) &           .7250(.0500) &           .7489(.0773) &  \textbf{.7739(.0924)} &  .8239(.0626) &  .8750(.1118) \\
     36 &           .6975(.0724) &  \textbf{.7449(.0762)} &           .6902(.0828) &           .5771(.0238) &           .5870(.0661) &           .6442(.0705) &           .5200(.0400) &           .5690(.0674) &           .5400(.0374) &           .5652(.0465) &           .5587(.0198) &  .8427(.0281) &  .9400(.0583) \\
     37 &           .5514(.0630) &           .5263(.0600) &  \textbf{.5541(.0643)} &           .5167(.0333) &           .5333(.0408) &           .5301(.0425) &           .5000(.0000) &           .5167(.0333) &           .5000(.0000) &           .5333(.0408) &           .5328(.0413) &  .7917(.0331) &  .9833(.0333) \\
     38 &           .7406(.1110) &           .8167(.0915) &           .7542(.1141) &           .7097(.0932) &  \textbf{.8569(.0588)} &           .7934(.0823) &           .7247(.0121) &           .8045(.0563) &           .7580(.0243) &           .6535(.0919) &           .7118(.0786) &  .9854(.0042) &  1.000(.0000) \\
     39 &           .8463(.1996) &           .8463(.1996) &           .8463(.1996) &           .8463(.1996) &           .8463(.1996) &           .7427(.2217) &           .5000(.0000) &           .7981(.1876) &           .7500(.2236) &           .8463(.1996) &  \textbf{.8481(.2010)} &  .9209(.1024) &  .9500(.1000) \\
     40 &  \textbf{.8022(.0858)} &           .7970(.0843) &           .7893(.0837) &           .6411(.0792) &           .6945(.0516) &           .7618(.0949) &           .6119(.0719) &           .6690(.0728) &           .6258(.0820) &           .5840(.0295) &           .5700(.0631) &  .9064(.0721) &  .9714(.0571) \\
\hline
   Mean &           .8062(.0608) &  \textbf{.8174(.0640)} &           .8058(.0608) &           .7577(.0475) &           .7751(.0512) &           .7968(.0604) &           .6923(.0388) &           .7579(.0586) &           .7478(.0586) &           .7431(.0520) &           .7532(.0524) &  .8960(.0298) &  .9900(.0120) \\
\hline
Wilcox &                         1 &                   .99736 &                  .782792 &                 .0024846 &                 .0937058 &                  .136656 &               $9.15 \times e^{-7}$ &                .00105434 &               $9.68 \times e{-5}$ &               $3.86 \times e^{-5}$ &                 .0001961 &                1 &                1 \\
 Wilcox &                         NA &                         - &                         = &                         + &                         = &                         = &                         + &                         + &                         + &                         + &                         + &                - &                - \\
Wilcox &                .00282207 &                         1 &                 .0184106 &                .00031885 &                .00683614 &                .00376574 &               $2.82 \times e^{-7}$ &               $3.76 \times e^{-5}$ &               $4.86 \times e^{-6}$ &                $1.78 \times e^{-5}$ &               .000138562 &                1 &                1 \\
 Wilcox &                         + &                         NA &                         + &                         + &                         + &                         + &                         + &                         + &                         + &                         + &                         + &                - &                - \\
\hline
\end{tabular}
}
\end{center}
\end{table}
\end{landscape}
\restoregeometry

